LinkTeller: Recovering Private Edges from Graph Neural Networks via Influence Analysis

Graph structured data have enabled several successful applications such as recommendation systems and traffic prediction, given the rich node features and edges information. However, these high-dimensional features and high-order adjacency information are usually heterogeneous and held by different data holders in practice. Given such vertical data partition (e.g., one data holder will only own either the node features or edge information), different data holders have to develop efficient joint training protocols rather than directly transfer data to each other due to privacy concerns. In this paper, we focus on the edge privacy, and consider a training scenario where Bob with node features will first send training node features to Alice who owns the adjacency information. Alice will then train a graph neural network (GNN) with the joint information and release an inference API. During inference, Bob is able to provide test node features and query the API to obtain the predictions for test nodes. Under this setting, we first propose a privacy attack LinkTeller via influence analysis to infer the private edge information held by Alice via designing adversarial queries for Bob. We then empirically show that LinkTeller is able to recover a significant amount of private edges, outperforming existing baselines. To further evaluate the privacy leakage, we adapt an existing algorithm for differentially private graph convolutional network (DP GCN) training and propose a new DP GCN mechanism LapGraph. We show that these DP GCN mechanisms are not always resilient against LinkTeller empirically under mild privacy guarantees ($\varepsilon>5$). Our studies will shed light on future research towards designing more resilient privacy-preserving GCN models; in the meantime, provide an in-depth understanding of the tradeoff between GCN model utility and robustness against potential privacy attacks.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> changes.tex <==
\clearpage
\newpage

\begin{center}
    \vspace{1em}
    \huge\sffamily\bfseries
    Summary of Changes
    \vspace{1em}
\end{center}

\setcounter{subsection}{0}
\setcounter{page}{1}

We would like to thank all reviewers for their constructive and insightful feedback. We conducted additional experiments and improved the writing of the paper following the suggestions. In this letter, we list our revision details corresponding to reviewers' comments.
\begin{enumerate}
    \item Reviewers’ comments in \textit{\textbf{black}, italic font};
    \item General discussions and concrete changes in black font (all changes are in \textcolor{blue}{blue} font in the attached paper body).
\end{enumerate}
We address the list of \textit{expected changes} provided in the revision feedback below.
% ; we then address \textit{individual comments} from each reviewer in Section~\ref{sec-A2}.

% \subsection{Expectations for Revision}
% \label{sec-A1}
\vspace{0.5cm}
\setcounter{expectation}{0}

\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Stealthiness)}: 
\textit{Discuss alternative detection strategies which would reduce the number of queries used in the attack (perhaps at the cost of performance, \eg, Precision). }
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We have pointed out the stealthiness issue and alternative detection strategies in~\Cref{sec:dp-bound} and concretely discussed the details in~\Cref{sec:append-stealthy}.

In particular, we describe details of potential detection strategies as follows. First, a defender can use validation data to evaluate both the attack and benign query performance in terms of the attack F1-score and query node classification accuracy under different query limits. 
Then the defender could optimize a query limit $Q$ which decreases the attack performance while maintaining reasonable benign query accuracy. Such a query limit would depend on the properties of different datasets and how safety-critical the application is. Note that in general limiting the number of queries will not affect the performance for a single user, while it would hurt if several users aim to query about the same set of nodes, thus the query limit could be made for each node. In practice, the defender can directly flag the users who try to exceed the query limit $Q$ for a limited set of nodes as suspicious for further inspection.


\vspace{0.5cm}
\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Choice of parameters)}: 
\textit{Ensure that all parameters are selected during validation and final performance determined during testing.}
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We have followed the suggestion to select the privacy parameter $\varepsilon$ based on the validation set, and then report the final performance on the testing set.
The results are added to~\Cref{sec:eval-dp-util} and~\Cref{sec:append-choice}.

Basically, when selecting $\varepsilon$ on the \textit{validation set}, we set a lower threshold for the model utility, and select the smallest $\varepsilon$ satisfying the condition that the utility of the trained DP-GCN on the validation set is higher than the given threshold. (One example threshold is the F1-score of the MLP model.) Then, we evaluate both the model utility and attack success rate under the selected $\varepsilon$ on the \textit{testing set}.

We additionally point out that the added results serve as the supplementary result to our current results in~\Cref{fig:dp-attack} and analysis in~\Cref{sec:eval-dp-util} and~\Cref{sec:tradeoff}, where we aim to show the existence of a tradeoff between model utility and privacy, as well as the dependencies of the tradeoff, which are interesting and novel ﬁndings of the work.

\vspace{0.5cm}
\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Density belief)}: 
\textit{Discuss actionable strategies for the attacker given limited knowledge of the density $k$ and/or strategies to improve the accuracy of the density belief. Tone down claims that estimation of $k$ is unimportant and frame the discussion with respect to the observed Precision and Recall rather than the broad performance across all $\hat{k}$s.}
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We completely agree and appreciate that the reviewers point this out. $k$ is indeed important and our previous observation was that overall it is not too sensitive. We have:

\begin{enumerate}
    \item toned down the claim that the estimation of $k$ is unimportant and presented finer-grained discussions, as suggested, for Precision and Recall rather than overall performance in~\Cref{sec:attack-eval}.
    \item provided discussion on the actionable strategies for the attacker given limited knowledge of the density $k$ and/or strategies to improve the accuracy of the density belief in~\Cref{sec:oracles} and~\Cref{sec:append-belief}. For example, the attacker could use some similar publicly available graphs (\eg, a similar social network) or partial graphs to estimate $k$. Specifically:
    \begin{enumerate}
        \item The attacker could estimate $k$ based on partial graph information (as suggested by Reviewer A). With the prior knowledge of some connected/unconnected pairs, the attacker can calculate the inﬂuence values for each known pair. Then, she can estimate a threshold for distinguishing the connected pairs from the unconnected ones with high conﬁdence, and thus obtain the estimated density belief $\hat k$.
        \item The attacker could estimate $k$ based on the relationship of one or a few particular nodes (as suggested by Reviewer C). The attacker can start from an intentionally low $\hat k$ and increase it until an edge is inferred for the relationship, or until the known existing edges are inferred. The attacker then stops at this specific $\hat k$ and takes it as the density belief.
        \item The attacker could estimate $k$ by running a link prediction algorithm. When a partial graph is available, the attacker can run a link prediction algorithm, \eg, training a link prediction model, to predict all edges in the graph. Based on the predictions, the attacker will then obtain a rough estimate of the density belief $\hat k$ for use in \linkteller.
    \end{enumerate}
\end{enumerate}

\vspace{0.5cm}
\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Attacker capabilities)}: 
\textit{Discuss how the attack might change in settings where the attacker's capabilities are stronger or weaker. For example, where they have additional knowledge of some edges or can only control a subset of node features.}
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We have discussed the variations of our attack under different settings of various attacker capabilities in~\Cref{sec:oracles} and~\Cref{sec:append-capable}, with a focus on the two settings outlined by the reviewers.

\ul{When the attacker has additional knowledge of some edges}: The attacker’s prior knowledge on the existence of some edges can be leveraged to improve the density belief $\hat k$ in our \linkteller. More concretely, based on the knowledge of some edges, the attacker can calculate their inﬂuence values. Then, she can estimate a threshold for distinguishing the edges from the unconnected pairs with high conﬁdence, and then obtain a refined estimation of the density belief $\hat k$. The attack effectiveness will subsequently be improved.

\ul{When the attacker has only partial control over a subset of node features}: We thank Reviewer A for clarifying the setting. In this setting, part of the feature information is lost, and thus the accuracy of the estimation of the influence value would be negatively impacted, leading to the decrease of attack performance. However, how much the attack effectiveness will degrade also depends on the importance of the missing features.

\vspace{0.5cm}
\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Other architectures)}: 
\textit{Clarify that the GAT experiment evaluates the \textit{transferability} of the attack from a GCN. Reason about the performance in this setting and outline the limitations that future work must overcome to adapt \linkteller to other architectures. }
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We have followed the reviewers’ suggestion and clarify the goal of our GAT experiment on \textit{transferability} and provide more discussion about its performance in~\Cref{sec:attack-gat}, as detailed below. 

The GAT experiment mainly aims to investigate the \textit{transferability} of our inﬂuence analysis based attack from GCNs, as both of them perform information propagation guided by the graph structure. However, since the structures of GCNs and GATs are diﬀerent, the exact inﬂuence calculation for the two models shall be diﬀerent (one related to the graph convolution, the other related to the attention mechanism). As revealed by the experiment, the inﬂuence calculation is indeed not directly generalizable, leading to the lower attack performance of \linkteller on GAT, and interestingly, it is still much higher than baseline methods.

We have also added the discussion on the limitations to overcome in adapting \linkteller to other architectures in~\Cref{sec:append-limit}. First and foremost, in order to achieve high attack effectiveness, we need to derive exact inﬂuence calculations for diﬀerent GNN structures specifically. We believe that our influence analysis based framework has the potential to perform well on diﬀerent GNN structures with the inﬂuence value calculation tailored to each of them. Another potential obstacle in the adaptation is that \linkteller cannot deal with randomized models, such as the aggregation over sampled neighbors in GraphSAGE~\cite{hamilton17graphsage}. It could be an interesting future work to take such randomness into account for inﬂuence calculation.

\vspace{0.5cm}
\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Hard labels)}: 
\textit{Discuss how the attack might be adapted when logits are not available (as included in the rebuttal). }
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We have added the discussion in~\Cref{sec:append-capable} which focuses on the variations of the settings. We explain that it is not straightforward to adapt our \linkteller to handle the case where logits are not available, which belongs to the “decision based blackbox attack category” rather than the score based. There are a few works~\cite{brendel2017decision,dong2019efficient} in the image domain that perform certain decision-based blackbox attacks. However, how to estimate the gradient/inﬂuence value in GNNs based on decision remains an interesting future direction.

\vspace{0.5cm}
\stepcounter{expectation}
\noindent \textbf{Expectation \theexpectation} 
\textbf{(Baselines)}: 
\textit{Provide more clarity on the reasons for the poor performance of the baselines. }
\vspace{0.2cm}

\noindent \underline{\textbf{Response}:} 
We have added more clarifications for the poor performance of the baselines and conducted additional experiments to compare \linkteller with baselines in trasductive setting in~\Cref{sec:attack-eval} and~\Cref{sec:append-baseline-cmp}.

First of all, we note that LSA-X~\cite{he2020stealing} relies on measuring certain distances based on either posteriors (of the node classiﬁcation model) or node attributes to predict the connections. However, node classiﬁcation and edge inference (i.e., privacy attack goal here) are two distinct tasks, and node features (or posteriors) are useful for node classiﬁcation does not mean that they will be useful for edge inference. Thus, LSA-X which tries to provide the attacker with diﬀerent levels of node information as prior knowledge to perform the edge re-identiﬁcation attack is not eﬀective. On the contrary, \linkteller tries to analyze the inﬂuence between nodes, which reﬂects the edge connection information based on our theoretical analysis (\Cref{thm:k-layer-gcn}) and is indeed more eﬀective for edge inference as we show empirically.

We point out that, to our best knowledge, there are no such settings where \linkteller may fail but other existing approaches (\eg, LSA-X) may succeed. The detailed reasons are provided above. To summarize, our \linkteller leverages the edge influence information, which is more relevant for the task of edge re-identification attack than purely node level information used in LSA-X and we have add the discussion in~\Cref{sec:append-baseline-cmp}. We then discuss the two specific scenarios outlined by the reviewers.

\ul{If the model makes inferences on single nodes and not subgraphs}: In this case, \linkteller cannot obtain influence information between nodes of interests, and thus the edge re-identification performance would be less effective. Similarly for the baselines, where they would fail to calculate the statistics of a set of nodes to compare their similarity. That is to say, if the model makes inferences on single nodes, both \linkteller and baselines may fail to effectively attack, while \linkteller may still outperform baselines given that it leverages the influence value of edges explicitly.

% \linkteller cannot be expected to attain reasonable attack effectiveness, since it relies on calculating a bunch of influence values for all the pairs among the node set, sorting the pairs by their influence values and thus differentiating the connected ones from the unconnected. If there are only very few pairs, the value distribution may not be reliable. 
% The same also applies to LSA-X. Thus, in this case, the performance of both \linkteller and LSA-X will be hurt, and there is a high chance that \linkteller is still better than LSA-X given that \linkteller leverages the influence value of edges specifically.

\ul{If the inference is transductive vs. inductive}: We first point out that the inductive setting is more challenging than the transductive setting, where the inference nodes are already included in the training graph. We then analyze the potential performance of \linkteller in the transductive setting. \linkteller is naturally applicable to the transductive setting. Since these nodes are involved in model training, the influence value and the rank may be more accurate, leading to even better attack performance. Thus, we expect that \linkteller will achieve better performance in the transductive setting and retain its advantage over LSA-X.

We have conducted additional experiments as shown in~\Cref{sec:append-trans} comparing \linkteller to LSA-X using the datasets and evaluation protocols from He \etal~\cite{he2020stealing}, and we show that \linkteller still outperforms the baselines in the trasductive setting.



\iffalse
\subsection{Responses and Revisions to  Detailed Reviews}
\label{sec-A2}

\fan{the responses here in Section B are not reflected in the revision yet--we can discuss and decide whether and what to include}

\subsubsection{General Response}~\\
% \vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Threat Model:}
Does the threat model *require* Bob to supply part of the training data (the nodes) or is this just to show the typical setting? The attack itself seems to start at inference time (RA, RB, RC, RD).
\begin{itemize}[leftmargin=*]
    \item[--] If so, how much control over the nodes does Bob need? (RA)
    \item[--] Are there variations of this threat model for which the attack would still succeed (e.g., partial knowledge of edges) (RA)? 
    \item[--] If possible, can the authors give more real-world instantiations of this threat model (RA, RC, RD)? 
\end{itemize}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewers for the helpful question and suggestions.
We clarify that indeed the threat model does not require Bob to supply training data. We are sorry for the confusion, and we will update our paper by using another agent to provide the training data instead of Bob.
In particular, the GNN model can be trained using local data or data provided by \textit{any} user, and then deployed as a cloud service with a blackbox API exposed to users.
% The user Bob, as an adversary, only needs to provide the information (\ie, node features) of interested nodes during testing (attack) time. 
\begin{itemize}[leftmargin=*]
    \item[--] Bob only needs the node features of the set of nodes that he is interested in during inference.
    \item[--] Indeed, if the attacker has partial knowledge w.r.t. the existence of some edges, this prior knowledge can actually be leveraged to improve the process of \linkteller.
Assuming Bob has the prior knowledge of some connected/unconnected pairs, 
after calculating the influence value for each pair, 
he can obtain a distribution of the influence values, and thus estimate the threshold for distinguishing the connected pairs from the unconnected ones with high confidence.
In another word, such prior knowledge can help to estimate the \textit{density belief} in our algorithm, leading to potentially more successful attack.
    \item[--] 
    We first provide the abstract example. In our threat model, Alice and Bob could belong to different departments of the same company and Alice provides API access to other departments by training models with their (social) connection data, and she cannot transfer such connection data due to privacy concerns. If Bob is adversarial, he is particularly interested in the relationship between some nodes (\eg, product, personnel) out of personal interest, and thus conduct the privacy attacks to inference certain edge connections.

    % Aware of the possibility of mounting such an attack with low cost, Bob may well attempt at performing the attack.

We then refer to some real-world instantiations. 
On one hand, in particular, the similar vertically data split setting in graph data is also discussed in Zhou \etal~\cite{zhou2020privacy}.
On the other hand, our work is inspired
by one realistic scenario from our 
industrial collaborations, which we will 
include in the revised version of this paper. Specifically, a large Internet company that
we work with has two divisions, one
focuses on recommendations and another focuses on financial services. One division 
has data about user interactions (the graph)
while the other division has more features and labels about a user. For policy reason, one cannot copy data across division boundaries, and can only happen in a differentially private way. In this case, one division becomes
Alice and the other becomes Bob.
This is one real-world  
instantiation of our setting.





In addition, nowadays there are several ML/AI services/platforms that take the training data from users and help them to train  ML models as  queryable APIs, such as Vertex AI~\cite{VertexAI} from Google Cloud,  ParlAI platform~\cite{ParlAI} from Facebook AI, and  InfoSphere Virtual Data Pipeline~\cite{InfoSphe} from IBM. 
Thus, against these real-world cloud services, such threat model could lead to potential privacy concerns or even severe consequences.


\end{itemize}


\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Parameters:} 
The attack is somewhat sensitive to the parameters. 
\begin{itemize}[leftmargin=*]
    \item[--] Results regarding the best parameters (e.g., privacy budget) are obtained by analyzing test data, is it expected that practitioners could obtain similar performance by calibrating on validation data? (RB) 
    \item[--] The Precision-Recall tradeoff seems highly dependent on $k$, would an attacker be able to take action on the output of the attack despite the high variance here? (RC)
\end{itemize}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewers for the insightful question. 
\begin{itemize}[leftmargin=*]
    \item[--]
    We provide clarifications on the privacy parameter $\eps$ from the following two aspects.
    \underline{First}, 
one of our initial goals on such trade-off evaluation is to investigate and present the existence of such a trade-off, 
as well as its dependence on the dataset type (\eg, whether and how much the graph structure helps) and the degree distribution of the interested nodes (\eg, low degree nodes); the existence of the trade-off and its dependencies are interesting and novel findings of this work.
\underline{Second},
determining parameters via a validation dataset and evaluating the parameters on the testset can be expected to give similar performance, since the validation dataset and the testset are in similar distributions. 
There is one case where the practitioner might suffer a performance degradation---when the graph is very sparse, the validation set may not be able to provide good insights on the performance on the test set.
Otherwise, it is expected that practitioners could obtain similar performance by calibrating on validation data, and we will follow the suggestion to conduct experiments in our revision.
    \item[--]
    Regarding the density belief parameter $\hat k$, from our evaluation in Table I (under the worst case where the attacker has no knowledge about $k$), we can see that even wrong belief $\hat k$ (\eg, $\hat k=k/4$ or $4k$) provides reasonable attack success rate (far outperforming the baselines).
    On top of that, with some prior knowledge on the existence of some edges, 
    we can allow the attacker to achieve better attack performance by first estimating the density belief $\hat k$ via calculating the influence value for each known pair and obtaining the value distribution.
% assuming Bob has the prior knowledge of some connected pairs and unconnected pairs, 
% after calculating the influence value for each pair, 
% he can obtain a distribution of the influence values for the connected/unconnected pairs, and thus estimating the threshold for distinguishing them with high confidence.
In another word, the attacker can achieve reasonable attack performance without any knowledge of $k$, while the attack can be further improved by leveraging certain prior knowledge to estimate $\hat k$.

\end{itemize}


\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Baselines:} 
Are the authors able to elaborate on why the baselines (LSA-X, etc) perform so poorly? (RB, RC)

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewers for the helpful question. 
First, 
we note that LSA-X~\cite{he2020stealing} rely on measuring certain distances based on either posteriors (of the node classification model) or node attributes to predict the connections.
% we would like to clarify that the presented results of MLP represent the model's performance on node classification \emph{not} the performance of the attack.
However, node classification and edge inference (\ie, privacy attack goal here) are two distinct tasks, and node features (or posteriors) are useful for node classification does not mean that they will be useful for edge inference. 
Thus, LSA-X which tries to provide the attacker with different levels of node information as prior knowledge to perform the edge re-identification attack is not very effective. On the contrary, \linkteller tries to analyze the influence between nodes, which reflects the edge connection information based on our theoretical analysis (Theorem 1) and is indeed more effective for edge inference as we show empirically in~\Cref{tab:att-np} and~\Cref{tab:att-np-auc}. 

We provide some additional evidence that supports the point that node features may not be very useful for edge inference.
On some of the datasets (\eg, twitch-\{DE, ENGB\} and PPI), the performance of MLP (relying only on node features) are quite good, 
indicating that 
the gains from incorporating \textit{graph structures} into the node classification task are marginal, 
further implying the weak correlation between node features and the graph structure.
Thus, node feature information is far from sufficient in the edge inference task, which also explains the poor performance of LSA-X~\cite{he2020stealing}.
We will make these discussions more clear in our revision.




\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Stealthiness:} 
While the runtime of the attack is small, do the authors agree that the number of queries may become quite high, which would make the attack easier to detect? Can they imagine potential mitigation strategies given this observation? (RB)

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the interesting question and suggestion.
We agree that the number of queries will become quite high in the case when the attacker has a \textit{large} set of interested nodes (and thus inference nodes), since the query number is equal to $|V^{(I)}|$ in our algorithm.

Following the suggestion, we believe it is possible to evaluate the precision of the {attack} depending on the size of 
$V^{(I)}$ and $V^{(C)}$ to understand the impact of the number of attempts on the attack. If such impact is significant, we can potentially check the distribution of query numbers of different users and  identify the adversaries who may query specific nodes with high frequency. We will add the discussion in our revision.




\subsubsection{Reviewer A} ~\\
% \vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{The scenario in which the adversary knows and provides the node features for training the GNN may have somewhat limited applicability. Can you add more discussion about possible real-world instantiations of this scenario?}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the question.
We want to clarify that in our interaction model, we only need the \textit{users} to provide training information (\ie, node features), but such information does not need to come from the \textit{adversary}. The adversary only needs to provide the information of interested nodes during testing (attack) time. We will make our setting more clear in the revision.

Nowadays there are several ML/AI services/platforms that take the training data from  users and help users to train an ML model based on the provided data.
Vertex AI~\cite{VertexAI} from Google Cloud is such a unified platform that can help users train a built-in algorithm against their provided datasets without requiring the users to write a training application~\cite{vertexai-train-overview}.
They provide easy-to-use services, APIs, and client libraries that facilitate the process~\cite{vertexai-train-api}.
The ParlAI platform~\cite{ParlAI} from Facebook AI as well as the InfoSphere Virtual Data Pipeline~\cite{InfoSphe} from IBM also provide similar services.
Our interaction model is an abstraction of these prevalent ML services.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:} 
\textit{Can the setting be broadened in some way e.g. giving the attacker only partial control over the nodes, or control over only some of the nodes? Can it be adapted to settings in which the adjacency matrix takes values in the range [0,1] to indicate different strengths of the connection?}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the thoughtful comment and suggestions.
For the \underline{first} suggestion, we would like to clarify that the attacker does not have full control over all nodes. In fact, in the inference stage, Bob only queries the set of nodes that he has control over and is interested in by passing in the features of these nodes.
For the \underline{second} suggestion: Yes, both the GCN model and our \linkteller can be easily extended to the case of weighted adjacency matrix.
In terms of GCN, several works~\cite{liu2019higher,zhou2020weighted} have specifically studied weighted GCNs to account for connections of different strength (\eg, higher order connections).
Regarding our \linkteller, the real-valued weighted adjacency matrix will directly translate into our influence value calculation.
We will add related discussion in the paper.
% Thus, this adaptation is direct, and in this paper we only focus on the simple and widely used setting of 0/1 adjacency matrix to demonstrate the feasibility of our \linkteller attack.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Does the attack change if the attacker already knows some of the edges? If so, could this be used to improve the process of inferring edges e.g., once the attacker is sufficiently certain that there is an edge between nodes u and v, adjusting the influence matrix accordingly to account for this?}


\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the excellent point.
Indeed, the prior knowledge of the attacker w.r.t. the existence of some edges can be further leveraged to improve the process of \linkteller.
% We next discuss a straightforward potential approach.
For instance, assuming Bob has the prior knowledge of some connected pairs and unconnected pairs, 
after calculating the influence value for each pair, 
he can obtain a distribution of the influence values for the connected/unconnected pairs, and thus estimating the threshold for distinguishing the connected pairs from the unconnected ones with high confidence.
In another word, such prior knowledge can help to estimate the \textit{density belief} in our algorithm, leading to a potentially more successful attack, and we will add related discussion in the paper.
% With more knowledge, the estimation of the threshold will be more accurate, leading to a more successful attack.
% The suggestion from the reviewer of ``adjusting the influence matrix accordingly to account for this'' is also a valid approach worth considering and further refining.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Minor points including the abbreviation (GCN) and the typos (Alice and twitch-DE).}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for pointing them out. We will make corresponding updates in the revision.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Section 5F: the performance on GATs is described as ``slightly lower'' than on GCNs, but the differences between Tables 1 and 3 looks quite significant.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for pointing it out. 
Indeed, we will update our description to be precise.
We explain the differences between Table 1 (attack performance against GCNs) and Table 3 (attack performance against GATs) as follows.
Since the structures of GCNs and GATs are different, the exact influence calculation for the two models shall be different (one related to the graph convolution, the other related to the attention mechanism).
In our experiment, we directly apply \linkteller with the influence calculation derived on GCNs to GATs, aiming to evaluate the \textit{transferability} of our influence analysis based attack.
As revealed by the experiment, the influence calculation is not directly generalizable, and it is an interseting future work to derive the influence calculations for different GNN structures.
In the revision, we will adjust our statement and add the above discussion.

% ============================================================================================================
\vspace{0.5cm}
\subsubsection{Reviewer B}~\\
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{For instance, a \textbf{more detailed evaluation of the number of GNN layers} would be interesting.}


\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the helpful suggestion.
We have provided results for $2$-layer GCNs in Section V-E and $3$-layer GATs in Section V-F in the main paper, as well as results for 3-layer GCNs and analysis of $1$-layer and more than $3$-layer GCNs in Appendix E2.
In the revision, we will add additional evaluations on GNN with more layers and add corresponding analysis of the number of GNN layers.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Moreover, I am somewhat torn by the described setting: While the authors argue for a ``jointly trained'' model, the setting, as a matter of fact, describes a remotely deployed model with a user querying inputs. As the adversary is not using the knowledge of the training data, there is no need to consider this more complex and maybe more ``exotic'' scenario.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for pointing this out.
Sorry for this confusion in our interaction model: Indeed, we do not need the adversary to have knowledge of training data. We will make 
this clear in our revision by introducing another user who provides the training data, rather than using the same user ``Bob".
% and we will ma
% We agree with the reviewer that the model can indeed be viewed as a remotely deployed model with a user querying inputs, and the adversary indeed does not need the knowledge of training data to perform the attack.
% We will make the modifications accordingly in our revision.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{The proposed attack queries the same set of testing samples $V^{(I)}$ multiple times ($n=|V^{(C)}|$) with one sample slightly altered to infer the relations among the nodes (in the presented experiments $|V^{(I)}|=|V^{(C)}|=500$). This significantly increases the number of queries conducted by the adversary, which, in turn, may allow to detect the attack easily.  
The authors give this a casual brush-off by stating that the runtime of the attack is relatively small (tens of seconds according to Table VIII in Appendix E-4). While this might be acceptable in this specific scenario, I want to motivate the authors to \textbf{discuss alternative detection strategies based on the queries themselves}. For instance, one could evaluate the precision of the attack depending on the size of $V^{(I)}$ and $V^{(C)}$.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the comment.
We will follow the suggestion to discuss alternative detection strategies.
Following the suggestion, we would evaluate the precision of the {attack} depending on the size of 
$V^{(I)}$ and $V^{(C)}$ to understand the impact of the number of attempts on the attack. If such impact is significant, we can potentially check the distribution of query numbers of different users and  identify the adversaries who may query specific nodes with high frequency. We will add the discussion in our revision.


In addition, we apologize for the typo in the evaluation section, where  $V^{(I)}$ should be replaced by $V^{(C)}$, and $|V^{(I)}|>|V^{(C)}|=500$. 
Concretely, 
for the twitch datasets, the set of inference nodes are all nodes in each test graph; for PPI and Flickr, we will add the detailed split (training/validation/testing) in dataset statistics in Table IV.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{\textbf{What is the influence of the dataset?} According to the presented experiments, the used datasets can be learned with MLPs as well. The F1 scores lie within 0.06 (Flicker) or less (*Please use equal ranges for the plots in Figure 3a*). The flicker dataset is also the one where the attack performs worst. Moreover, LSA-X has been evaluated on completely different datasets. For the sake of transparency, it would be great to have these datasets analyzed as well.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the comments and helpful suggestions.
We summarize the following properties of the dataset that will influence the F1 score and attack performance:
1) closeness of the training  and  testing graph in distribution;
2) sparsity of the graph.
In general, large difference in training and testing and severe sparsity of the graph will increase the difficulty of both training and attack.
For the poor performance on Flickr dataset, we provide an analysis at the end of Section V-E.
In short, given the highly sparse structure of the Flickr dataset, the trained GCN model on Flickr does not achieve good performance. This implies that the parameters of the trained network on this dataset may not capture the graph structure very well, and thus the attack performance is negatively influenced.
The sparsity also leads to the large variance in attack results which arises from node sampling.
We will follow the suggestion to use equal ranges for the plot.
Finally, we explain the distinction between the dataset selection in our paper and  the baseline LSA-X~\cite{he2020stealing}.
% \sout{, which arises from the difference in the learning setting---LSA-X focuses on the transductive setting while we focus on the more challenging and general inductive setting. Thus, we have to choose different datasets which are constructed for different settings.}
% \yh{I feel this may lead the reviewers to believe that we are applying LSA-X to a setting that they are not designed for. Could we say that ``LSA-X was evaluated on datasets designed for transductive setting`` instead of saying that the method focuses on transductive setting? Just curious, does our method also work on transductive setting? If so, we might consider adding some experiments in the revision to show that we can beat LSA-X under transductive setting as well? }
LSA-X was evaluated on datasets designed for \textit{transductive setting} while we focus on \textit{inductive setting} in our interaction model. Thus, we have to choose  datasets accordingly.
In fact, our \linkteller can also be generalized to transductive setting, and we will consider adding some experiments in our revision.
% The datasets in their setting are not suitable for our setting, 
% although the idea of their attack can be applied to our dataset.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{\textbf{What are alternative ways of defense next to DP?} For most applications, it probably is not necessary to communicate the logits through the remote API. When reading the paper, I was wondering what would be necessary to conduct a similar attack if only the final class $c$ would be reported or a rank of the top-x classes. In other words, what are the limits of the attack in a slightly different but equally practical scenario: not leaking logits.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the interesting question.
Yes, as \linkteller requires the logits outputs as query results,  reporting only the final class $c$ or a rank of top-x classes would be a potential defense against \linkteller.
% , and thus only communicating the logits through the remote API is indeed a possible defense against \linkteller.
In addition, in the case where only the final class $c$  or a rank of the top-x classes would be reported, it will require more queries to perform certain decision based blackbox attacks in image domain~\cite{dong2019efficient,brendel2017decision}, and how to estimate the gradient/influence value in graphs is  an interesting future direction.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{\textbf{Why is LinkTeller superior to LSA-X (He et al., 2021)} The authors briefly address this in Section V-E but do not go into much detail. For instance, they say that LSA does not work because it relies on posteriors or node attributes. However, judging by the presented results using MLP, it seems perfectly manageable to learn the data at hand without any additional graph-based data.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the interesting question. 
First, 
we would like to clarify that the presented results of MLP represent the model's performance on node classification \emph{not} the performance of the attack.
Node classification and edge inference (\ie, privacy attack goal here) are two distinct tasks, and node features are useful for node classification does not mean that they will be useful for edge inference. 
Thus, LSA-X which tries to provide the attacker with different levels of node information as prior knowledge to perform the edge re-identification attack is not very effective. On the contrary, \linkteller tries to analyze the influence between nodes, which would reflect the edge connection information based on our theoretical analysis (Theorem 1), and we show that such influence analysis is indeed effective for edge inference empirically.

In addition, the good performance of MLP (relying only on node features) on some datasets indicates that 
the gains from incorporating \textit{graph structures} into the node classification task are marginal, 
% graph structure does not help much in the node classification task, 
further implying the weak correlation between node features and the graph structure.
Thus, node features are far from sufficient in the edge inference task, which also explains the poor performance of LSA-X~\cite{he2020stealing}.
We will make these discussions more clear in our revision.
% In comparison, our \linkteller leverages the influence analysis which excludes a large number of negative samples (Theorem 1), thus attaining superior attack performance than LSA-X.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Finally, I would like to point the authors to their argumentation of choosing the correct parameters, such as the privacy budget $\epsilon$. In Section VI-D, ``Tradeoff between Model Utility and Privacy,'' it is suggested that it is possible to balance the individual objectives by inspecting the presented results. However, as these are determined on testing data (for which we do not have ground truth in practice), this is not possible but has to be done on validation data. That aspect can be easily fixed in the paper by more careful argumentation. However, I believe it would be worthwhile to demonstrate this in the experiments and \textbf{determine all parameters during validation (including $\epsilon$) and demonstrate performances with these on testing data}. This mimics reality as close as possible and would add a nice touch to the evaluation.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the suggestion. 
We will definitely check and make more careful argumentation in our revision.
One of our initial goals on the evaluation is to investigate and present the existence of such a trade-off, 
as well as its dependence on the dataset type (\eg, whether and how much the graph structure helps) and the degree distribution of the interested nodes (\eg, low degree nodes); the existence of the trade-off and its dependencies are novel findings of this work.
We will also follow the suggestion and will conduct experiments accordingly by determining parameters during validation and evaluating on the testset in our revision.




% ============================================================================================================

\vspace{0.5cm}
\subsubsection{Reviewer C}~\\
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{I think this is vital because the attacker doesn't know if their estimate is too high or too low, so they are not able to adjust their future actions based on the most likely outcome, i.e., they don't know if a particular edge is likely to be a true positive, whether they have many missing edges, or vice-versa, so it's difficult for them to act on the predictions. }

\textit{This could be improved by providing some actionable strategies for the attacker given limited knowledge of $k$. For example, if they're interested in a particular node relationship, can they start from an intentionally low $\hat{k}$ and increase it until an edge is inferred for this relationship. Then given the $\hat{k}$ at which the edge appears, can they estimate the likelihood of it being a true positive? }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the valuable suggestion. 
Indeed, we can allow the attacker to estimate the density belief $\hat k$ first for better attack performance. For instance, assuming Bob has the prior knowledge of some connected pairs and unconnected pairs, 
after calculating the influence value for each pair, 
he can obtain a distribution of the influence values for the connected/unconnected pairs, and thus estimating the threshold for distinguishing them with high confidence.
In another word, even with limited knowledge of $k$, the attacker can leverage prior knowledge as such to obtain the density belief $\hat k$ which leads to potentially more successful attack.
In addition, from our evaluation under the worst case where the attacker has no knowledge about $k$, we can see from Table I that even wrong belief $\hat k$ (\eg, $\hat k=k/4$ or $4k$) provides reasonable attack success rate (outperforming the baselines).
% We clarify that the exact prior knowledge of the existence of an edge is required so that the attacker can estimate the true positive rate.
% One actionable strategy given such kind of prior knowledge is described in the response to Comment 3 of Reviewer A.


% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Note that the attacker goals are tightly linked to $n^{(I)} = |V^{(I)}|$, so considering values other than 500 would be really beneficial here. }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the suggestion.
We will provide additional experimental results with values other than $500$ in the revision for the comprehensiveness of the evaluation.
Note that here we randomly picked the number 500 without any tuning and we \textit{randomly} sampled the set of nodes of interest for attack.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Also related to $k$: it's not clear what value is used for the setting in Table II which has extremely high AUC-PR. Presumably it was fixed at some value to fit the setting in prior work. }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the question.
We clarify that in the calculation of AUC-PR, the knowledge of $k$ is not required. 
Overall, the AUC-PR value gives an evaluation of the performance of a binary classifier under a series of $k$ (as explained below).
% \yh{Can we put the last sentence in this paragraph here? A high-level explanation before getting into the details seems more clear to me.}
Basically, to calculate AUC-PR, we only need the influence value of each connected/unconnected pair. Then, we can sort the pairs increasingly by their influence values. At each pair, we can compute a precision/recall value to obtain a PR curve. The AUC-PR value is thus the area under the PR curve.
% To summarize, the AUC-PR value gives an overall evaluation of the performance of a binary classifier under a series of $k$.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{The attack performance in some settings is quite low; namely for the Flikr dataset and when applied to the GAT—for which it is extremely low. In addition, the claim that ``LinkTeller has the potential to generalize to other GNNs'' seems unsubstantiated (§V.F). It's also noted that the ``influence based analysis does imply some fundamental common characteristics of GNNs which could lead to other future research'' (§V.F) but these common characteristics are not mentioned. }

\textit{I would consider this experiment a bonus result, but these statements should be toned down—although I think it could also be a really valuable opportunity to reason about these characteristics. Conceptually, why should LinkTeller generalize to other architectures like GAT? How does the information propagation manifest in different architectures? From LinkTeller's perspective, does the attention mechanism in GAT play a similar role to the convolutions in the GCN? The performance is considerably lower, why might this be? What are the limitations that future work must overcome to adapt LinkTeller to other architectures?  }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the comment and the thoughtful suggestions.
% We acknowledge that the attack performance for \linkteller on the Flickr dataset on the GAT model is low.
We will provide explanations from two aspects.
\underline{First}, the attack performance of \linkteller on the Flickr dataset  is not quite high, and we have analyzed the potential reason at the end of Section V-E. 
Basically, due to the highly sparse structure of the Flickr dataset, the trained GCN model does not achieve good performance, and thus the parameters of the trained network may not capture the graph structure very well, leading to the poor attack performance.
\underline{Second}, our goal of applying \linkteller to GAT is to investigate the generalizability of our influence analysis based attack, as both of them perform information propagation guided by graph structure.
% since  expect that 
% the attention mechanism in GAT plays a similar role to the convolutions in the GCN.
% This, basically, belong to the ``common characteristics of GNNs''---the information propagation guided by the graph structure. 

However, as revealed by the experimental results, 
a more exact influence calculation for the GAT model is needed to achieve high attack performance.
We believe that  \linkteller framework has the potential to perform well on different GNN structures with the influence value calculation  tailored to each of them. 
One potential limitation in adapting \linkteller to other architectures is that \linkteller cannot deal with randomized models, such as the aggregation over sampled neighbors in GraphSAGE~\cite{hamilton17graphsage}, which could be an interesting future work to take such randomness into account for influence calculation.
In the revision, we will add corresponding discussions.
% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Another aspect of the evaluation which could use deeper analysis is the performance of the baselines which all fail, almost universally. It would be really valuable to explore why this is the case. Is it wholly due to their assumption that shadow datasets or partial graphs are available or is it that including information about node influence makes all the difference? }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the suggestion.
In our opinion, it is indeed the influence that gives us the huge advantage over their method.
% More analysis regarding this can be found in the response to Comment 6 of Reviewer B.
% We will make it more clear in the revision.
We note that LSA2-\{post, attr\}~\cite{he2020stealing} rely on measuring certain distances based on either posteriors or node attributes to predict the connections.
However,
node classification and edge inference (\ie, privacy attack goal here) are two distinct tasks, and node features (or posteriors) are useful for node classification does not mean that they will  be useful for edge inference.
Thus, LSA2-\{post, attr\} is not very effective only leveraging these to perform the edge re-identification attack. 
In comparison, \linkteller tries to analyze the influence between nodes, which reflects the edge connection information based on our theoretical analysis (Theorem 1) and is indeed more effective for edge inference empirically.

We provide some additional evidence that supports the point that node features may not be very useful for edge inference.
On some of the datasets (\eg, twitch-\{DE, ENGB\} and PPI), the performance of MLP (relying only on node features) are quite good, 
indicating that 
the gains from incorporating \textit{graph structures} into the node classification task are marginal, 
further implying the weak correlation between node features and the graph structure.
Thus, node features are far from sufficient in the edge inference task, which also explains the poor performance of LSA2-\{post, attr\}~\cite{he2020stealing}.
We will make these discussions more clear in our revision.



% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{It doesn't seem that the LinkTeller attack requires the attacker to also provide the training nodes. Is it the case that the attacker can actually recover private edges from any pretrained cloud-based GCN (for example)? This would be a much stronger and more compelling attack.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the comment. We do not need to assume that the attacker provides the training data. 
% \yh{A nit, \textit{``yes, we do not ...``} is not common in English, can we delete the \textit{yes} here?} 
The attacker can actually recover private edges from any pretrained cloud-based GCN by querying the set of nodes of interest.
 We will make this clear in our revision.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{I might have missed something, but in the evaluation there is no $V^{(C)}$, only $V^{(I)}$, is it correct to assume that in the evaluation $V^{(C)} = V^{(I)}$ (i.e., all of the inference nodes are of interest)?}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We are sorry for the typo and we clarify that all $V^{(I)}$ in the evaluation section should be  $V^{(C)}$. In fact, $V^{(C)}$ is a subset sampled from $V^{(I)}$.
Concretely, for the twitch datasets, $V^{(I)}$ is the set of all nodes in each test graph; for PPI and Flickr, we will add the detailed split (training/validation/testing) in dataset statistics in Table IV.
$V^{(C)}$ is the subset of $V^{(I)}$ sampled following different criteria in terms of the node degree distribution.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{It's stated that ``$V$ can be a union of nodes in a group of graphs, as long as the grouping makes logical and practical sense'' (§III.A). Is this just describing a typical setting or is it an actual assumption required by the attack? }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We are sorry for the confusion.
% Yes, \yh{\textit{yes} is not necessary here as the question is about \textit{A or B} rather than \textit{yes or no}} 
Here we aim to describe a typical scenario in the inductive setting. We will consider removing the notation $V$ for clarity, since $V^{(T)}$ and $V^{(I)}$ are already sufficient for denoting the training and inference graph.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{It's stated that ``the attacker has no information about the API model except that it is a GNN model with unknown architecture and parameters'' (§III.B), however the attacker does also know the node training data. This is clear in context but should be explicit here.  }

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the comment.
This comment and the response are in fact associated with that in Comment 6. 
The attacker does not need to know the training data. Only the information about the blackbox API and the features of nodes targeted by the attacker is sufficient for the attacker to carry out the attack.
We will modify relevant parts in the revision to make this more clear.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{In §IV.A I think it would be beneficial to give some quick intuition about why EdgeRand and LapGraph are differentially private when they're first mentioned here, or at least provide a forward pointer to their in-depth descriptions in §IV.B as the motivation of this subsection hinges on the DP guarantees of the perturbation methods.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the thoughtful suggestion and will add the discussion on the intuitions in the revision. Concretely, both \edgerand and \lapgraph are differentially private due to the perturbation of the adjacency matrix. The perturbation guarantees that the probability of getting the same perturbed matrix is close for two adjacency matrices differing by one edge. Specifically, \edgerand flips each entry in the adjacency matrix independently with a probability determined by the privacy budget. \lapgraph adds Laplacian noise to the adjacency matrix and uses the noisy density estimation to clip each entry of the adjacency matrix into 0 or 1. We will add these discussions in our revision.
% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{It would be useful if the y-axes of Figs. 3 and 4 were to the same scale, just to allow easier comparison between datasets.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the suggestion and will adjust the y-axes of the figures accordingly in the revision.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{As the values $d_{low}$ and $d_{high}$ are chosen ``empirically'' it would be useful to mention what kind of reasoning was used to pick them (§V.D).}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the question.
We choose nodes of different degrees to provide a more comprehensive evaluation of the performance of \linkteller under different scenarios (i.e., nodes of interest are of low/high degrees).
The values $d_{\rm low}$ and $d_{\rm high}$ are chosen by examining the node degree distribution of each specific graph.
We select the two values such that the total number of nodes with degree $\leq d_{\rm low}$ (or $\geq d_{\rm high}$) are of roughly similar scale.
For example, twitch datasets contain graphs of thousands of nodes and the node degree distribution is relatively more concentrated, so we pick the two values to be $5$ and $10$.
The consideration for some special cases such as twitch-PTBR, PPI, and Flickr are more concretely explained at the end of Section V-D.

% =======================================

\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Other abbreviations, typos, and statements.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for pointing them out, and we will update all of them in the revision.

% ============================================================================================================


\vspace{0.5cm}


\subsubsection{Reviewer D}~\\
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{Although I do understand the scenario/threat model the authors describe,
how realistic is it really for Bob to perform adversarial queries
against Alice's trained model to infer private information that wouldn't
have been ``copied'' over in the first place due to privacy concerns?
(The assumption and the concern here is that Bob and Alice belong to the
same company and while I do see why Alice won't be sharing information
due to privacy concerns, I do see less likely Bob performing such an
attack due to ethics and liability.) Don't get me wrong: the attack still
exists, and so does the vulnerability. It would however be more
convincing if the authors could clarify this further with real examples.}

\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the question.
We refer to Zhou \etal~\cite{zhou2020privacy} for the vertically data split setting in graph data where each data holder holds partial node features and their own edges.
In particular, we would like to first give an \textit{abstract} example of our threat model---Alice and Bob belong to different departments of the same company. Alice provides API access to other departments of the company. Bob is particularly interested in the relationship between some nodes (\eg, product, personnel) out of personal interest. 
% Aware of the possibility of mounting such an attack with low cost, Bob may well attempt at performing the attack.
% We provide additional discussions w.r.t. the interaction model and the threat model.

In \textit{real-world scenarios}, there are several ML/AI services/platforms that take the training data from users and help users to train an ML model based on the provided data, such as Vertex AI~\cite{VertexAI} from Google Cloud, the ParlAI platform~\cite{ParlAI} from Facebook AI, and the InfoSphere Virtual Data Pipeline~\cite{InfoSphe} from IBM. Our interaction model is an abstraction of these prevalent ML services.
In our interaction model particularly, 
we only need the \textit{users} to provide training information (\ie, node features), but such information does not need to come from the adversary. The \textit{adversary} only needs to provide the information of interested nodes during testing (attack) time.
We will make our setting more clear in the revision by introducing another user who provides the training data other than ``Bob''.

% We also acknowledge Comment 1 from Reviewer A, Comment 2 from Reviewer B, and Comment 6 from Reviewer C regarding the setting, and will make adjustments accordingly in our revision.


\vspace{0.5cm}
\stepcounter{comment}
\noindent \textbf{Comment \thecomment:}
\textit{In Section III.A, the authors mention that ``[...] during the inference
stage, Bob will collect node features of the inference graph $X^{(I)}$
(e.g., patients in the next months). What guarantees do we have that
$X^{(I)}$ does not introduce non-stationarity that would affect the
performance of the underlying model to start with? That might affect the
attack somehow although I don't have any intuition on how nor severity.
However, I am also assuming this to not really be a problem as that
would otherwise affect the underlying performance of the model and it
should have been quite visible to the authors.}


\vspace{0.2cm}
\noindent \textbf{\underline{Response:}} 
We thank the reviewer for the thoughtful comment.
We would like to clarify that the task of the underlying model (\eg, public API) is to perform the node classification on the selected nodes $V^{(I)}$, while an adversary aims to infer the private edge connection information via such queries. That is to say, the performance of the underlying model is related with the inference node selection but would be less likely to be largely affected since the attacker did not manipulate any information.
We will make the discussion clear in our revision.

% The selection of $V^{(I)}$ will affect the performance of the blackbox API.
% Subsequently, the attack performance will inevitably be affected.
% The results on Flickr is a good example that possibly falls into this case, as concretely discussed at the end of Section V-E. 

\fi



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/tab_attack_dp_full.tex <==
{

\setlength{\tabcolsep}{4pt} % column sep

\begin{table}
    \centering
    \caption{twitch-RU (\edgerand)}
    \label{tab:att_dp_twitch-RU-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 1.3 & 1.9 & 1.3 & 1.9 & 1.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 1.5 & 2.1 & 3.0 & 4.3 & 6.2 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 4.8 & 6.7 & 5.1 & 7.3 & 4.0 & 3.3 & 3.3 & 1.9 & 2.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.5 & 2.1 & 3.0 & 4.3 & 4.8 & 3.7 & 7.7 & 4.2 & 12.8 & 6.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 19.0 & 6.7 & 12.8 & 3.6 & 9.3 & 1.9 & 8.0 & 2.8 & 6.7 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.2 & 2.1 & 7.7 & 1.7 & 11.0 & 2.0 & 18.7 & 6.2 & 31.5 & 15.1\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 28.6 & 11.7 & 25.6 & 13.1 & 17.3 & 10.0 & 16.7 & 4.7 & 16.7 & 2.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.5 & 3.9 & 16.0 & 8.3 & 20.8 & 11.9 & 39.9 & 13.2 & 78.9 & 12.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 38.1 & 17.8 & 38.5 & 10.9 & 38.7 & 7.5 & 34.0 & 1.6 & 20.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 12.8 & 6.0 & 24.0 & 7.9 & 46.1 & 11.5 & 80.3 & 8.2 & 97.0 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 71.4 & 11.7 & 56.4 & 3.6 & 57.3 & 5.0 & 39.3 & 1.9 & 21.3 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.7 & 4.4 & 34.5 & 2.1 & 67.4 & 6.1 & 92.7 & 7.4 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.2 & 6.7 & 79.5 & 3.6 & 73.3 & 1.9 & 42.0 & 3.3 & 21.3 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 31.5 & 4.0 & 48.6 & 3.0 & 86.4 & 5.9 & 98.5 & 2.1 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.7 & 0.1 & 0.6 & 0.1 & 1.2 & 0.4 & 1.6 & 0.6 & 1.5 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.2 & 0.0 & 0.3 & 0.1 & 1.3 & 0.4 & 3.4 & 1.3 & 6.4 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 1.5 & 2.1 & 1.3 & 2.3 & 1.2 & 2.1 & 0.7 & 2.1 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.3 & 0.4 & 1.2 & 0.7 & 2.5 & 1.3 & 4.5 & 1.6 & 9.2 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 5.2 & 4.3 & 5.8 & 2.6 & 7.2 & 1.8 & 6.4 & 1.7 & 6.4 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 1.1 & 3.1 & 1.3 & 7.8 & 1.7 & 13.8 & 3.1 & 27.8 & 5.3\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 5.5 & 2.7 & 7.5 & 2.2 & 9.0 & 2.0 & 11.6 & 2.0 & 15.4 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.5 & 0.7 & 4.0 & 1.0 & 9.7 & 1.7 & 25.2 & 3.6 & 66.9 & 7.4\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 9.2 & 3.9 & 12.4 & 3.1 & 21.1 & 3.2 & 30.9 & 3.6 & 20.3 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.5 & 1.0 & 6.7 & 1.4 & 22.9 & 2.8 & 67.2 & 5.3 & 88.6 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 22.1 & 4.5 & 36.2 & 4.4 & 45.1 & 2.8 & 36.5 & 1.5 & 21.2 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.0 & 0.9 & 19.7 & 1.6 & 49.2 & 1.0 & 79.7 & 1.6 & 92.5 & 1.0\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 55.1 & 2.4 & 61.9 & 2.9 & 55.7 & 3.2 & 39.8 & 1.5 & 22.3 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.0 & 0.4 & 33.8 & 0.4 & 60.8 & 1.5 & 86.8 & 0.6 & 97.1 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 72.1 & 6.4 & 75.6 & 5.0 & 66.5 & 3.1 & 43.2 & 1.9 & 22.5 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.7 & 1.2 & 41.3 & 1.5 & 72.6 & 1.2 & 94.2 & 0.2 & 98.3 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 87.5 & 1.9 & 85.9 & 1.7 & 70.5 & 2.2 & 43.5 & 1.7 & 22.5 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.9 & 0.8 & 47.0 & 1.1 & 77.0 & 2.2 & 94.9 & 1.4 & 98.2 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 91.9 & 3.3 & 86.9 & 0.9 & 70.8 & 2.3 & 43.0 & 2.0 & 22.5 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 1.2 & 47.5 & 1.6 & 77.3 & 2.0 & 93.7 & 1.5 & 98.0 & 0.7\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering     \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 15.6 & 9.1 & 11.2 & 4.6 & 9.2 & 3.7 & 7.1 & 2.5 & 5.5 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.8 & 1.4 & 4.0 & 1.4 & 6.6 & 2.2 & 10.2 & 3.0 & 15.7 & 3.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 22.3 & 11.9 & 15.5 & 5.8 & 12.4 & 3.0 & 11.3 & 2.2 & 10.0 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.0 & 1.9 & 5.6 & 1.7 & 9.0 & 1.6 & 16.4 & 2.1 & 28.9 & 2.5\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 27.5 & 7.7 & 25.3 & 4.9 & 24.6 & 5.4 & 22.6 & 3.2 & 20.3 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.0 & 1.1 & 9.2 & 1.3 & 17.8 & 2.7 & 32.9 & 2.6 & 59.2 & 3.7\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 38.7 & 8.9 & 36.9 & 5.9 & 37.6 & 4.5 & 39.4 & 3.4 & 29.8 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.0 & 1.3 & 13.5 & 1.8 & 27.4 & 1.8 & 57.4 & 1.3 & 86.9 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 55.9 & 5.4 & 57.5 & 3.3 & 59.6 & 2.5 & 56.1 & 2.9 & 32.2 & 2.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.2 & 0.7 & 21.0 & 0.7 & 43.6 & 1.7 & 81.9 & 2.9 & 93.8 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 71.9 & 2.9 & 76.8 & 1.6 & 78.1 & 2.2 & 59.1 & 4.2 & 32.7 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.1 & 0.6 & 28.1 & 1.5 & 57.1 & 2.6 & 86.2 & 1.5 & 95.4 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 88.1 & 2.1 & 88.7 & 1.5 & 86.0 & 2.1 & 61.9 & 3.7 & 33.5 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.1 & 0.8 & 32.5 & 1.8 & 63.0 & 3.2 & 90.3 & 1.2 & 97.6 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 94.0 & 0.8 & 93.5 & 0.5 & 88.4 & 1.7 & 63.4 & 3.5 & 33.8 & 2.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.2 & 1.2 & 34.3 & 2.3 & 64.7 & 3.4 & 92.6 & 1.7 & 98.5 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 96.8 & 0.3 & 95.6 & 0.8 & 89.0 & 1.9 & 63.3 & 3.8 & 33.7 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.7 & 1.3 & 35.0 & 2.4 & 65.2 & 3.3 & 92.4 & 1.1 & 98.4 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 97.5 & 0.4 & 96.3 & 0.3 & 89.4 & 1.7 & 62.8 & 4.2 & 33.5 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.9 & 1.3 & 35.3 & 2.5 & 65.5 & 3.7 & 91.6 & 1.3 & 97.8 & 0.4\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage

\begin{table}
    \centering
    \caption{twitch-RU (\lapgraph)}
    \label{tab:att_dp_twitch-RU-lap}
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.8 & 2.5\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 5.3 & 5.0 & 4.0 & 3.3 & 2.3 & 2.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 5.9 & 5.4 & 8.8 & 7.1 & 10.3 & 8.9\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 7.7 & 6.3 & 6.7 & 1.9 & 5.3 & 2.5 & 4.3 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 4.5 & 3.7 & 7.7 & 1.7 & 12.2 & 5.3 & 19.8 & 6.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 23.8 & 24.3 & 20.5 & 13.1 & 14.7 & 5.0 & 12.0 & 3.3 & 9.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.8 & 7.6 & 12.2 & 7.6 & 16.9 & 5.0 & 27.8 & 6.4 & 45.1 & 2.3\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 28.6 & 20.2 & 25.6 & 7.3 & 21.3 & 3.8 & 21.3 & 4.1 & 16.3 & 3.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.3 & 6.3 & 15.4 & 3.4 & 24.8 & 2.7 & 49.7 & 7.1 & 75.9 & 9.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 42.9 & 20.2 & 30.8 & 12.6 & 32.0 & 8.6 & 28.7 & 5.0 & 18.0 & 2.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 14.0 & 6.2 & 18.4 & 6.9 & 36.9 & 7.6 & 66.8 & 8.0 & 83.9 & 8.9\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 52.4 & 13.5 & 48.7 & 3.6 & 48.0 & 6.5 & 36.7 & 2.5 & 19.7 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.2 & 4.1 & 29.8 & 2.6 & 56.1 & 5.3 & 86.2 & 5.7 & 92.4 & 7.3\\
\bottomrule
    \end{tabular}%
}
\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 1.8 & 0.7 & 1.8 & 0.4 & 1.2 & 0.2 & 0.9 & 0.1 & 0.7 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.5 & 0.2 & 1.0 & 0.2 & 1.3 & 0.2 & 2.0 & 0.3 & 2.9 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 3.9 & 0.1 & 3.1 & 0.4 & 2.4 & 0.7 & 1.4 & 0.4 & 1.0 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.1 & 0.1 & 1.7 & 0.3 & 2.6 & 0.9 & 3.1 & 1.1 & 4.5 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 6.4 & 1.6 & 7.6 & 1.3 & 5.9 & 0.7 & 3.4 & 0.5 & 2.1 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.7 & 0.4 & 4.2 & 0.7 & 6.5 & 0.9 & 7.5 & 1.4 & 9.1 & 1.5\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 12.4 & 2.6 & 13.2 & 1.6 & 13.1 & 1.5 & 7.6 & 0.8 & 4.3 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.4 & 0.6 & 7.2 & 0.7 & 14.3 & 1.9 & 16.6 & 2.1 & 19.0 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 18.3 & 0.8 & 26.9 & 2.0 & 24.2 & 0.8 & 14.8 & 1.1 & 8.3 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.0 & 0.2 & 14.7 & 0.5 & 26.5 & 1.7 & 32.5 & 3.5 & 36.3 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 35.5 & 3.4 & 43.0 & 3.4 & 39.1 & 1.3 & 25.5 & 1.0 & 14.4 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.7 & 0.7 & 23.5 & 1.1 & 42.6 & 0.9 & 55.6 & 2.6 & 62.9 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 50.8 & 8.8 & 57.3 & 4.9 & 50.5 & 2.4 & 32.3 & 1.9 & 17.8 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.8 & 2.1 & 31.2 & 1.9 & 55.1 & 1.5 & 70.6 & 1.4 & 77.8 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 64.7 & 7.6 & 65.8 & 3.8 & 57.1 & 2.3 & 36.5 & 1.5 & 19.7 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.7 & 1.9 & 35.9 & 0.6 & 62.3 & 0.2 & 79.7 & 0.1 & 85.8 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 71.9 & 4.0 & 72.7 & 3.0 & 61.6 & 3.1 & 39.3 & 1.8 & 20.7 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.6 & 0.9 & 39.7 & 0.3 & 67.3 & 1.8 & 85.7 & 0.5 & 90.4 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 77.7 & 3.5 & 78.4 & 2.5 & 65.8 & 2.5 & 40.6 & 1.3 & 21.5 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.3 & 1.1 & 42.8 & 1.3 & 71.8 & 1.0 & 88.7 & 1.0 & 93.7 & 1.2\\
\bottomrule
    \end{tabular}%
}
\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 3.6 & 0.5 & 3.3 & 1.1 & 2.5 & 0.7 & 2.0 & 0.3 & 1.8 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.7 & 0.1 & 1.2 & 0.3 & 1.8 & 0.4 & 2.9 & 0.2 & 5.3 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 10.5 & 1.2 & 8.5 & 1.9 & 5.3 & 1.1 & 3.6 & 0.6 & 2.5 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.9 & 0.2 & 3.1 & 0.5 & 3.9 & 0.6 & 5.2 & 0.5 & 7.4 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 22.2 & 3.5 & 19.6 & 2.0 & 11.5 & 1.6 & 6.9 & 1.1 & 4.3 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.1 & 0.6 & 7.1 & 0.7 & 8.3 & 0.9 & 10.1 & 1.1 & 12.7 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 39.3 & 3.9 & 38.4 & 3.4 & 23.6 & 3.2 & 13.3 & 1.9 & 8.3 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.2 & 0.4 & 14.0 & 0.7 & 17.2 & 1.3 & 19.4 & 1.6 & 24.0 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 56.9 & 3.5 & 61.2 & 2.3 & 44.2 & 3.9 & 25.3 & 2.3 & 14.5 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.4 & 0.4 & 22.4 & 0.8 & 32.2 & 0.9 & 36.8 & 1.0 & 42.2 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 73.8 & 1.6 & 76.3 & 1.1 & 66.9 & 2.3 & 40.4 & 2.9 & 22.2 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.5 & 0.9 & 28.0 & 1.7 & 48.9 & 1.8 & 58.9 & 0.5 & 64.6 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 83.9 & 1.0 & 85.1 & 1.2 & 76.9 & 2.9 & 50.2 & 3.5 & 27.0 & 2.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.4 & 1.1 & 31.2 & 1.8 & 56.2 & 1.9 & 73.2 & 0.6 & 78.7 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 90.2 & 0.7 & 90.2 & 0.2 & 82.5 & 2.3 & 54.7 & 3.3 & 29.8 & 2.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.5 & 1.1 & 33.1 & 2.3 & 60.4 & 2.7 & 79.9 & 0.9 & 86.8 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 93.3 & 0.3 & 93.0 & 0.5 & 85.8 & 1.7 & 58.8 & 3.6 & 31.5 & 2.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.1 & 1.2 & 34.1 & 2.5 & 62.8 & 3.4 & 85.8 & 0.8 & 91.8 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.1 & 0.5 & 95.1 & 0.2 & 88.1 & 1.5 & 61.2 & 4.1 & 32.5 & 2.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.4 & 1.2 & 34.9 & 2.5 & 64.5 & 3.6 & 89.3 & 0.6 & 94.9 & 0.2\\
\bottomrule
    \end{tabular}%
}
\end{subtable}
\end{table}
\newpage

\begin{table}
    \centering
    \caption{twitch-DE (\edgerand)}
    \label{tab:att_dp_twitch-DE-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.6 & 3.6 & 1.3 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 5.6 & 7.9 & 5.6 & 7.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 16.7 & 23.6 & 8.3 & 11.8 & 4.2 & 5.9 & 2.2 & 3.1 & 4.4 & 4.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.8 & 6.7 & 4.8 & 6.7 & 4.8 & 6.7 & 4.8 & 6.7 & 18.7 & 17.3\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 25.0 & 20.4 & 17.9 & 12.7 & 21.7 & 11.8 & 23.2 & 13.6 & 16.7 & 5.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.5 & 5.9 & 10.3 & 7.4 & 24.2 & 12.4 & 49.2 & 28.2 & 69.8 & 23.4\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 41.7 & 31.2 & 31.0 & 8.4 & 35.8 & 12.8 & 32.9 & 11.5 & 22.7 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.1 & 10.2 & 18.7 & 4.6 & 40.1 & 13.1 & 69.8 & 23.4 & 95.2 & 6.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 83.3 & 23.6 & 66.7 & 23.6 & 54.0 & 11.1 & 44.4 & 4.2 & 23.8 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 26.2 & 7.0 & 40.1 & 13.1 & 60.7 & 10.5 & 94.4 & 7.9 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 3.9 & 4.8 & 2.3 & 2.2 & 1.4 & 1.0 & 1.2 & 0.4 & 1.1 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.0 & 1.2 & 1.2 & 1.2 & 1.4 & 1.0 & 2.3 & 0.8 & 4.3 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 5.7 & 6.6 & 3.7 & 3.6 & 3.2 & 0.9 & 2.8 & 0.5 & 2.7 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 1.7 & 1.8 & 1.9 & 3.1 & 1.1 & 5.4 & 0.7 & 10.2 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 6.4 & 6.3 & 5.1 & 3.5 & 5.3 & 2.0 & 5.6 & 1.6 & 6.0 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.6 & 1.6 & 2.5 & 1.8 & 5.1 & 2.1 & 10.5 & 2.6 & 22.5 & 4.7\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 8.9 & 5.3 & 9.0 & 4.6 & 10.1 & 2.0 & 9.4 & 0.9 & 11.6 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.2 & 1.4 & 4.4 & 2.5 & 9.7 & 2.3 & 17.9 & 0.8 & 43.9 & 2.5\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 12.4 & 4.9 & 16.5 & 2.0 & 19.4 & 2.7 & 23.3 & 1.1 & 23.3 & 2.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.0 & 1.4 & 7.9 & 1.2 & 18.5 & 2.3 & 44.4 & 1.5 & 88.1 & 3.9\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 27.7 & 4.6 & 33.7 & 1.5 & 40.4 & 4.9 & 42.2 & 5.1 & 24.6 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.6 & 1.2 & 16.1 & 0.4 & 38.3 & 2.5 & 79.9 & 4.8 & 93.2 & 2.4\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 55.7 & 8.6 & 60.1 & 5.8 & 61.8 & 7.4 & 46.6 & 4.6 & 25.4 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.3 & 2.3 & 28.7 & 1.6 & 58.6 & 2.9 & 88.3 & 2.9 & 96.4 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 73.0 & 3.5 & 77.1 & 2.4 & 71.7 & 6.5 & 48.1 & 4.3 & 25.7 & 2.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.5 & 1.8 & 36.9 & 1.5 & 68.2 & 2.9 & 91.3 & 2.2 & 97.5 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 84.8 & 1.8 & 84.6 & 4.4 & 77.2 & 6.7 & 48.5 & 4.0 & 25.5 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.3 & 1.0 & 40.4 & 1.1 & 73.5 & 4.5 & 92.1 & 1.6 & 97.0 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 88.3 & 1.5 & 90.2 & 3.8 & 80.2 & 5.6 & 49.1 & 4.6 & 25.6 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.1 & 1.1 & 43.2 & 1.5 & 76.4 & 3.2 & 93.2 & 2.3 & 97.3 & 0.6\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 3.6 & 2.4 & 3.1 & 0.9 & 2.9 & 0.7 & 2.4 & 0.2 & 2.5 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.9 & 0.6 & 1.6 & 0.5 & 3.0 & 0.8 & 4.9 & 0.5 & 10.3 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 7.2 & 2.0 & 6.0 & 1.1 & 6.0 & 0.5 & 5.9 & 0.7 & 5.6 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.8 & 0.5 & 3.1 & 0.7 & 6.1 & 0.6 & 12.1 & 1.9 & 22.8 & 3.8\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 12.9 & 0.8 & 11.6 & 1.4 & 12.4 & 0.4 & 13.0 & 0.1 & 12.4 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.3 & 0.3 & 5.9 & 1.0 & 12.6 & 0.8 & 26.4 & 1.1 & 50.3 & 3.8\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 20.2 & 2.2 & 21.0 & 0.9 & 23.3 & 0.9 & 23.9 & 0.8 & 20.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.2 & 0.7 & 10.7 & 1.0 & 23.7 & 2.0 & 48.6 & 3.9 & 82.3 & 2.7\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 34.6 & 1.4 & 38.6 & 1.8 & 43.1 & 1.9 & 42.0 & 0.9 & 23.1 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.8 & 0.7 & 19.7 & 1.9 & 43.8 & 3.9 & 85.3 & 3.8 & 93.6 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 52.5 & 1.9 & 59.5 & 0.9 & 68.0 & 0.9 & 44.7 & 2.0 & 24.0 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.4 & 0.9 & 30.2 & 1.6 & 69.0 & 4.2 & 90.7 & 2.0 & 97.1 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 75.5 & 3.3 & 80.0 & 1.6 & 75.9 & 0.9 & 45.8 & 1.7 & 24.2 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.2 & 1.8 & 40.6 & 2.7 & 77.1 & 3.6 & 92.8 & 1.2 & 97.9 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 89.1 & 3.3 & 90.1 & 1.9 & 77.9 & 0.3 & 46.3 & 1.4 & 24.2 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.7 & 1.9 & 45.8 & 3.2 & 79.1 & 3.6 & 93.8 & 2.0 & 98.0 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 95.1 & 0.3 & 93.0 & 1.3 & 78.4 & 0.7 & 46.3 & 2.0 & 24.0 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.2 & 1.1 & 47.2 & 2.9 & 79.5 & 3.5 & 93.8 & 0.8 & 97.0 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 97.7 & 1.0 & 95.6 & 0.3 & 79.1 & 1.4 & 46.6 & 1.8 & 24.3 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.8 & 1.0 & 48.5 & 2.5 & 80.3 & 2.9 & 94.4 & 1.2 & 98.3 & 0.4\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{twitch-DE (\lapgraph)}
    \label{tab:att_dp_twitch-DE-lap} 
    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}   
    \multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.7 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.8 & 3.9\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.7 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 11.1 & 7.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 3.1 & 6.2 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 4.8 & 6.7 & 26.2 & 7.0\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 5.1 & 7.3 & 8.8 & 2.3 & 7.3 & 2.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 5.6 & 7.9 & 18.7 & 4.6 & 31.0 & 10.8\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 8.3 & 11.8 & 4.8 & 6.7 & 5.1 & 7.3 & 13.7 & 5.0 & 11.8 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.8 & 3.9 & 2.8 & 3.9 & 5.6 & 7.9 & 29.0 & 10.2 & 49.6 & 11.5\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 8.3 & 11.8 & 23.9 & 8.1 & 21.1 & 5.2 & 18.2 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 5.6 & 7.9 & 27.0 & 9.0 & 44.8 & 10.3 & 76.6 & 10.8\\
\bottomrule
    \end{tabular}%
}
\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 0.9 & 0.7 & 0.3 & 0.9 & 0.3 & 0.8 & 0.5 & 0.6 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.3 & 0.2 & 0.3 & 0.1 & 0.9 & 0.4 & 1.5 & 0.8 & 2.3 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 2.5 & 1.3 & 2.0 & 0.9 & 1.9 & 0.8 & 1.4 & 0.7 & 1.0 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.6 & 0.3 & 0.9 & 0.4 & 1.7 & 0.6 & 2.6 & 1.1 & 3.7 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 6.4 & 1.7 & 5.7 & 1.3 & 4.8 & 0.6 & 3.0 & 0.5 & 1.8 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.5 & 0.3 & 2.7 & 0.4 & 4.6 & 0.2 & 5.7 & 0.6 & 7.0 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 11.0 & 1.8 & 12.2 & 2.6 & 12.3 & 1.5 & 7.3 & 0.8 & 4.0 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.6 & 0.4 & 5.8 & 0.9 & 11.6 & 0.6 & 13.8 & 0.7 & 15.1 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 17.4 & 3.3 & 21.5 & 3.7 & 26.7 & 3.1 & 16.5 & 1.9 & 8.6 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.2 & 0.9 & 10.2 & 1.6 & 25.3 & 1.6 & 31.4 & 2.4 & 32.5 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 30.1 & 4.8 & 36.0 & 3.7 & 40.1 & 3.3 & 26.4 & 1.9 & 14.2 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.2 & 1.2 & 17.2 & 1.1 & 38.2 & 2.0 & 50.2 & 2.2 & 54.0 & 2.3\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 41.8 & 5.7 & 50.4 & 5.1 & 54.0 & 3.6 & 35.2 & 2.5 & 19.4 & 1.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.0 & 1.0 & 24.0 & 1.2 & 51.4 & 0.3 & 67.0 & 1.5 & 73.8 & 2.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 54.3 & 3.8 & 61.5 & 1.8 & 61.2 & 4.1 & 40.2 & 2.6 & 21.9 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.0 & 1.3 & 29.5 & 1.9 & 58.2 & 0.6 & 76.5 & 0.7 & 83.3 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 66.3 & 2.7 & 72.3 & 4.6 & 68.1 & 6.6 & 44.2 & 3.6 & 23.8 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.9 & 1.0 & 34.5 & 0.4 & 64.7 & 2.0 & 84.0 & 1.6 & 90.4 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 73.8 & 3.9 & 78.0 & 3.7 & 73.4 & 7.2 & 46.8 & 3.4 & 24.6 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.6 & 0.3 & 37.3 & 0.8 & 69.8 & 2.4 & 89.0 & 0.5 & 93.4 & 1.1\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 2.1 & 1.0 & 1.9 & 0.6 & 1.6 & 0.5 & 1.3 & 0.3 & 1.1 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.5 & 0.2 & 1.0 & 0.3 & 1.6 & 0.4 & 2.6 & 0.6 & 4.5 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 5.5 & 1.3 & 5.2 & 0.4 & 3.2 & 0.2 & 2.2 & 0.0 & 1.6 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 0.4 & 2.7 & 0.2 & 3.2 & 0.1 & 4.4 & 0.2 & 6.3 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 13.7 & 1.4 & 12.7 & 0.3 & 7.6 & 0.3 & 4.3 & 0.3 & 2.6 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.5 & 0.5 & 6.5 & 0.5 & 7.8 & 0.6 & 8.7 & 0.9 & 10.6 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 26.1 & 1.2 & 26.2 & 0.7 & 15.4 & 1.1 & 8.5 & 0.5 & 4.8 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.6 & 0.6 & 13.3 & 0.5 & 15.6 & 0.4 & 17.2 & 0.3 & 19.5 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 38.9 & 2.0 & 47.1 & 1.7 & 31.4 & 1.8 & 17.3 & 1.2 & 9.5 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.9 & 0.9 & 24.0 & 2.0 & 31.8 & 0.2 & 34.9 & 0.7 & 38.6 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 58.1 & 3.1 & 66.4 & 2.9 & 50.1 & 2.2 & 27.9 & 1.3 & 15.2 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 14.8 & 1.4 & 33.8 & 2.9 & 50.8 & 2.0 & 56.6 & 1.7 & 61.7 & 2.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 73.9 & 1.7 & 77.6 & 0.5 & 63.4 & 2.0 & 36.2 & 1.7 & 19.2 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 18.8 & 1.1 & 39.4 & 2.2 & 64.4 & 2.4 & 73.3 & 1.4 & 77.7 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 84.5 & 1.0 & 85.2 & 1.3 & 68.0 & 1.5 & 39.9 & 1.0 & 21.0 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.5 & 1.3 & 43.3 & 2.7 & 69.0 & 2.5 & 80.9 & 2.1 & 85.1 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 90.7 & 1.8 & 88.9 & 0.7 & 73.7 & 1.2 & 42.6 & 1.4 & 22.4 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.1 & 1.5 & 45.1 & 2.3 & 74.7 & 2.5 & 86.4 & 1.6 & 90.6 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 94.0 & 0.3 & 92.6 & 0.7 & 76.1 & 1.4 & 44.4 & 1.9 & 23.2 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.9 & 1.2 & 47.0 & 2.5 & 77.2 & 2.7 & 90.0 & 0.8 & 94.1 & 0.6\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{twitch-FR (\edgerand)}
    \label{tab:att_dp_twitch-FR-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 6.7 & 9.4 & 3.3 & 4.7 & 1.7 & 2.4 & 4.4 & 2.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 3.3 & 4.7 & 3.3 & 4.7 & 3.3 & 4.7 & 17.5 & 8.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 5.0 & 4.1 & 8.6 & 3.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 10.0 & 8.2 & 34.2 & 15.9\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 6.7 & 9.4 & 6.7 & 9.4 & 15.6 & 6.3 & 19.2 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 3.3 & 4.7 & 6.7 & 9.4 & 30.8 & 13.0 & 75.0 & 4.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 38.9 & 7.9 & 28.3 & 8.5 & 32.5 & 3.5 & 35.6 & 7.5 & 25.6 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.8 & 1.2 & 14.2 & 4.2 & 32.5 & 3.5 & 70.0 & 16.3 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 77.8 & 15.7 & 80.0 & 16.3 & 71.7 & 2.4 & 49.4 & 3.4 & 25.6 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.7 & 2.4 & 40.0 & 8.2 & 71.7 & 2.4 & 96.7 & 4.7 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 7.1 & 7.2 & 3.8 & 3.4 & 2.5 & 2.0 & 1.8 & 1.0 & 1.5 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.7 & 1.8 & 1.8 & 1.7 & 2.4 & 1.9 & 3.4 & 2.1 & 5.5 & 2.6\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 9.1 & 9.4 & 5.4 & 4.8 & 4.5 & 3.1 & 3.7 & 1.9 & 3.6 & 1.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.2 & 2.3 & 2.6 & 2.4 & 4.3 & 3.1 & 6.9 & 3.9 & 13.5 & 5.3\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 11.2 & 10.3 & 9.1 & 6.1 & 8.1 & 4.2 & 9.1 & 2.8 & 9.6 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.7 & 2.5 & 4.3 & 3.0 & 7.7 & 4.3 & 17.0 & 5.7 & 35.9 & 11.2\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 15.0 & 12.7 & 16.7 & 5.4 & 17.0 & 4.9 & 18.7 & 4.0 & 18.3 & 2.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.6 & 3.1 & 7.8 & 2.8 & 16.0 & 5.0 & 35.0 & 8.2 & 68.2 & 11.7\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 21.0 & 10.1 & 23.9 & 7.6 & 29.1 & 6.5 & 36.0 & 3.5 & 24.5 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.0 & 2.6 & 11.3 & 3.9 & 27.3 & 7.0 & 67.2 & 8.6 & 91.0 & 3.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 41.5 & 6.2 & 47.9 & 6.3 & 57.7 & 4.6 & 46.4 & 1.8 & 25.5 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.7 & 1.8 & 22.4 & 3.7 & 53.8 & 6.0 & 86.4 & 3.5 & 94.9 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 63.2 & 4.1 & 68.1 & 3.8 & 69.6 & 3.8 & 48.9 & 1.7 & 25.9 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 14.8 & 1.3 & 31.8 & 2.8 & 64.8 & 5.3 & 90.9 & 2.5 & 96.4 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 83.1 & 3.9 & 84.0 & 3.5 & 76.8 & 3.2 & 49.8 & 1.9 & 26.1 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.4 & 1.4 & 39.2 & 2.5 & 71.5 & 2.5 & 92.5 & 1.2 & 97.2 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 90.4 & 1.2 & 91.5 & 0.9 & 82.2 & 3.9 & 51.0 & 2.4 & 26.3 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.1 & 0.8 & 42.6 & 1.1 & 76.5 & 2.3 & 94.8 & 1.7 & 97.8 & 0.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 94.6 & 0.3 & 92.6 & 1.3 & 82.4 & 2.7 & 51.1 & 1.9 & 26.6 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.1 & 0.8 & 43.2 & 1.3 & 76.7 & 1.6 & 94.9 & 0.9 & 98.8 & 0.4\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 4.6 & 4.2 & 3.7 & 2.4 & 3.4 & 0.9 & 3.2 & 1.0 & 3.2 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.1 & 1.1 & 1.8 & 1.2 & 3.3 & 1.0 & 6.4 & 2.4 & 12.5 & 2.9\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 8.7 & 2.4 & 8.5 & 2.5 & 8.5 & 3.2 & 8.1 & 2.4 & 7.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.1 & 0.7 & 4.2 & 1.5 & 8.5 & 3.7 & 15.9 & 5.9 & 30.1 & 6.6\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 14.9 & 1.6 & 18.3 & 1.0 & 19.2 & 0.2 & 18.2 & 0.4 & 16.8 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.6 & 0.5 & 8.8 & 0.5 & 18.6 & 1.5 & 35.3 & 2.8 & 65.0 & 5.1\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 31.8 & 3.0 & 32.6 & 2.2 & 32.2 & 0.4 & 32.9 & 0.3 & 21.9 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.8 & 1.3 & 15.8 & 1.9 & 31.2 & 2.3 & 63.7 & 5.6 & 84.7 & 6.4\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 45.3 & 2.5 & 49.6 & 4.1 & 53.9 & 1.1 & 44.2 & 1.4 & 24.0 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 11.0 & 1.5 & 24.2 & 3.8 & 52.3 & 5.5 & 85.5 & 5.1 & 92.6 & 4.3\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 65.0 & 1.6 & 71.7 & 0.2 & 74.8 & 1.9 & 46.8 & 2.2 & 24.6 & 1.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.7 & 1.4 & 34.8 & 2.9 & 72.5 & 6.7 & 90.3 & 3.7 & 95.0 & 3.4\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 80.4 & 2.6 & 84.5 & 2.6 & 79.5 & 1.1 & 48.6 & 2.9 & 25.3 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.5 & 2.0 & 41.0 & 3.9 & 77.0 & 5.8 & 93.6 & 2.6 & 97.4 & 1.4\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 92.3 & 2.3 & 92.8 & 1.2 & 80.5 & 1.3 & 48.4 & 2.7 & 25.2 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.3 & 1.8 & 45.0 & 3.7 & 77.9 & 5.5 & 93.3 & 3.1 & 97.0 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 97.1 & 1.2 & 96.0 & 1.0 & 84.2 & 1.4 & 49.0 & 2.7 & 25.4 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.5 & 2.1 & 46.5 & 4.2 & 81.6 & 6.2 & 94.6 & 3.1 & 97.8 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 98.0 & 0.8 & 97.2 & 0.8 & 84.9 & 1.1 & 49.2 & 2.9 & 25.3 & 1.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.7 & 2.1 & 47.1 & 4.3 & 82.2 & 6.6 & 94.8 & 2.9 & 97.5 & 1.8\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{twitch-FR (\lapgraph)}
    \label{tab:att_dp_twitch-FR-lap}    
    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 4.2 & 5.9\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 3.1 & 1.9 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 4.2 & 5.9 & 7.5 & 5.4\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 4.2 & 5.9\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 3.3 & 4.7 & 3.9 & 2.8 & 1.9 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 3.3 & 4.7 & 7.5 & 5.4 & 7.5 & 5.4\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 11.1 & 15.7 & 6.7 & 9.4 & 3.3 & 4.7 & 5.6 & 4.2 & 3.6 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.3 & 4.7 & 3.3 & 4.7 & 3.3 & 4.7 & 10.8 & 8.2 & 14.2 & 4.2\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 22.2 & 31.4 & 13.3 & 18.9 & 10.8 & 8.2 & 5.6 & 4.2 & 5.3 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.7 & 9.4 & 6.7 & 9.4 & 10.8 & 8.2 & 10.8 & 8.2 & 20.8 & 7.2\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 6.7 & 9.4 & 13.3 & 12.5 & 8.3 & 6.2 & 9.7 & 2.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 3.3 & 4.7 & 13.3 & 12.5 & 16.7 & 12.5 & 38.3 & 10.3\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 11.1 & 15.7 & 6.7 & 9.4 & 6.7 & 9.4 & 13.3 & 10.3 & 15.8 & 6.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.3 & 4.7 & 3.3 & 4.7 & 6.7 & 9.4 & 26.7 & 20.5 & 62.5 & 27.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 6.7 & 9.4 & 16.7 & 12.5 & 22.2 & 11.7 & 20.6 & 3.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 3.3 & 4.7 & 16.7 & 12.5 & 44.2 & 23.8 & 80.8 & 15.3\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 1.8 & 0.3 & 2.1 & 0.4 & 2.0 & 0.4 & 1.4 & 0.2 & 1.1 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.4 & 0.1 & 1.0 & 0.2 & 1.9 & 0.5 & 2.7 & 0.6 & 4.0 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 3.8 & 0.8 & 4.3 & 1.4 & 4.1 & 0.9 & 2.7 & 0.3 & 1.6 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.9 & 0.2 & 2.0 & 0.7 & 3.8 & 1.0 & 5.0 & 0.6 & 6.0 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 7.5 & 0.8 & 7.7 & 2.2 & 10.0 & 0.8 & 6.1 & 0.1 & 3.4 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.8 & 0.2 & 3.6 & 1.2 & 9.3 & 1.1 & 11.4 & 0.4 & 12.7 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 15.1 & 5.6 & 17.9 & 4.8 & 18.6 & 2.8 & 12.2 & 0.4 & 6.6 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.6 & 1.5 & 8.4 & 2.5 & 17.4 & 3.2 & 22.8 & 1.3 & 24.5 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 23.5 & 9.0 & 29.0 & 7.2 & 35.7 & 3.1 & 22.9 & 0.5 & 12.3 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.5 & 2.3 & 13.6 & 3.8 & 33.3 & 4.0 & 42.6 & 1.4 & 45.7 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 35.8 & 8.4 & 47.0 & 6.6 & 51.3 & 4.1 & 33.4 & 0.4 & 18.0 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.4 & 2.3 & 22.0 & 3.8 & 47.8 & 5.0 & 62.1 & 1.6 & 67.2 & 2.5\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 52.8 & 6.5 & 62.3 & 6.0 & 62.6 & 3.2 & 40.1 & 0.9 & 21.4 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 12.4 & 1.9 & 29.1 & 3.6 & 58.4 & 4.2 & 74.7 & 1.8 & 79.7 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 66.9 & 5.9 & 73.3 & 4.5 & 69.6 & 2.8 & 43.8 & 1.8 & 23.6 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.7 & 1.8 & 34.2 & 3.1 & 64.8 & 3.4 & 81.5 & 1.5 & 87.6 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 78.1 & 4.2 & 81.1 & 1.9 & 74.1 & 1.2 & 46.9 & 1.3 & 24.6 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 18.3 & 1.6 & 37.8 & 2.1 & 69.0 & 3.1 & 87.3 & 2.2 & 91.6 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 85.3 & 1.4 & 85.9 & 1.9 & 77.3 & 2.0 & 48.2 & 1.6 & 25.3 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.9 & 1.0 & 40.1 & 2.1 & 72.0 & 2.7 & 89.7 & 2.2 & 94.0 & 0.7\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 3.0 & 1.0 & 3.2 & 1.2 & 2.7 & 0.7 & 2.4 & 0.3 & 1.7 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.7 & 0.2 & 1.5 & 0.4 & 2.6 & 0.4 & 4.5 & 0.4 & 6.6 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 7.8 & 0.6 & 8.4 & 0.9 & 5.3 & 0.7 & 3.5 & 0.6 & 2.6 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.9 & 0.0 & 4.1 & 0.2 & 5.1 & 0.2 & 6.7 & 0.5 & 9.8 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 16.3 & 1.2 & 17.3 & 0.8 & 10.8 & 1.4 & 6.2 & 0.8 & 3.9 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.9 & 0.3 & 8.3 & 0.4 & 10.3 & 0.4 & 11.8 & 0.5 & 14.8 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 30.2 & 0.6 & 33.9 & 1.4 & 22.9 & 1.7 & 12.9 & 1.3 & 7.4 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.3 & 0.7 & 16.4 & 0.8 & 22.1 & 0.6 & 24.7 & 0.5 & 28.5 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 47.0 & 1.9 & 54.0 & 2.4 & 42.6 & 2.6 & 23.7 & 2.1 & 13.0 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 11.4 & 1.1 & 26.2 & 2.7 & 41.1 & 1.2 & 45.5 & 0.5 & 50.0 & 1.4\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 67.9 & 2.5 & 73.1 & 0.9 & 60.0 & 0.9 & 33.9 & 1.8 & 18.4 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.5 & 1.8 & 35.4 & 3.1 & 58.1 & 4.1 & 65.4 & 2.3 & 70.9 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 79.8 & 3.8 & 83.4 & 1.7 & 71.4 & 2.0 & 41.0 & 3.2 & 21.6 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.3 & 1.9 & 40.4 & 3.3 & 69.0 & 4.1 & 78.9 & 1.0 & 83.2 & 1.5\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 87.7 & 2.9 & 89.5 & 1.6 & 74.7 & 1.5 & 43.7 & 2.5 & 22.8 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.3 & 2.0 & 43.4 & 3.9 & 72.4 & 5.5 & 84.2 & 2.5 & 88.0 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 91.5 & 2.1 & 91.9 & 1.4 & 78.0 & 1.0 & 46.0 & 2.4 & 23.8 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.1 & 1.8 & 44.6 & 4.2 & 75.7 & 7.3 & 88.7 & 3.1 & 91.7 & 2.3\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.0 & 0.9 & 93.9 & 1.5 & 80.2 & 0.6 & 46.7 & 2.5 & 24.4 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.0 & 2.0 & 45.5 & 4.5 & 77.7 & 6.0 & 90.1 & 3.0 & 93.9 & 2.1\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{twitch-ENGB (\edgerand)}
    \label{tab:att_dp_twitch-ENGB-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.7 & 0.9 & 2.3 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.7 & 2.4 & 8.4 & 3.1\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 8.3 & 11.8 & 4.8 & 6.7 & 2.6 & 3.6 & 3.3 & 0.9 & 5.0 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.1 & 2.9 & 2.1 & 2.9 & 2.1 & 2.9 & 6.3 & 1.1 & 19.7 & 4.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 13.1 & 10.2 & 19.4 & 6.5 & 18.2 & 3.5 & 14.7 & 1.9 & 9.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.2 & 3.2 & 10.5 & 3.7 & 18.5 & 4.4 & 29.8 & 8.7 & 39.5 & 12.3\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 13.1 & 10.2 & 22.0 & 5.9 & 18.4 & 10.1 & 16.0 & 3.3 & 14.0 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.8 & 2.7 & 11.7 & 3.0 & 20.1 & 14.2 & 32.7 & 12.3 & 58.4 & 24.2\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 56.0 & 13.8 & 46.5 & 12.8 & 37.7 & 5.4 & 33.3 & 3.8 & 20.7 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.9 & 4.5 & 26.1 & 9.8 & 39.5 & 12.3 & 67.7 & 18.9 & 81.9 & 13.2\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 60.7 & 10.5 & 58.6 & 2.1 & 54.6 & 1.0 & 41.3 & 1.9 & 26.0 & 4.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 18.0 & 1.9 & 31.9 & 6.2 & 55.9 & 10.8 & 81.9 & 13.2 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 83.3 & 11.8 & 82.8 & 4.1 & 74.1 & 3.4 & 46.7 & 6.8 & 26.0 & 4.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.6 & 6.9 & 44.6 & 5.2 & 75.6 & 14.0 & 90.7 & 6.7 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 1.5 & 0.8 & 0.7 & 0.5 & 0.4 & 0.6 & 0.5 & 0.4 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.4 & 0.5 & 0.5 & 0.4 & 0.7 & 0.5 & 1.5 & 1.2 & 2.2 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 1.5 & 1.3 & 1.0 & 1.3 & 0.8 & 0.9 & 0.2 & 0.7 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.3 & 0.5 & 0.7 & 0.6 & 1.3 & 0.5 & 1.9 & 0.4 & 3.3 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.8 & 1.1 & 1.2 & 0.9 & 1.5 & 0.6 & 1.9 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.5 & 0.7 & 1.5 & 1.1 & 3.6 & 1.8 & 8.7 & 4.5\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 2.1 & 2.0 & 1.6 & 1.7 & 3.2 & 1.3 & 3.3 & 1.0 & 4.5 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.7 & 0.7 & 1.0 & 1.1 & 3.8 & 1.9 & 7.8 & 3.4 & 20.7 & 8.3\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 3.7 & 0.8 & 4.8 & 1.1 & 8.1 & 0.7 & 11.2 & 1.2 & 13.5 & 3.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.1 & 0.4 & 2.5 & 0.1 & 9.1 & 2.6 & 25.1 & 7.9 & 61.8 & 24.3\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 15.2 & 2.6 & 16.5 & 0.9 & 22.9 & 3.2 & 27.2 & 3.7 & 20.1 & 3.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.1 & 0.3 & 9.0 & 1.7 & 25.9 & 8.7 & 61.2 & 19.9 & 84.3 & 6.4\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 30.5 & 3.0 & 38.3 & 5.0 & 40.1 & 4.7 & 34.3 & 3.8 & 21.2 & 4.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.3 & 1.2 & 21.6 & 6.7 & 44.4 & 12.3 & 73.3 & 9.8 & 88.6 & 5.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 58.4 & 4.6 & 56.4 & 2.0 & 52.3 & 3.2 & 38.4 & 5.3 & 22.7 & 5.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.2 & 3.9 & 31.1 & 7.4 & 56.5 & 10.0 & 81.6 & 9.1 & 94.3 & 2.8\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 77.9 & 2.7 & 71.3 & 2.9 & 61.3 & 3.6 & 41.8 & 7.7 & 23.1 & 5.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.5 & 4.3 & 39.0 & 8.6 & 66.4 & 12.0 & 87.9 & 6.9 & 95.6 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 79.5 & 1.4 & 77.9 & 3.4 & 64.7 & 5.8 & 42.7 & 9.4 & 23.1 & 5.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.9 & 4.5 & 42.4 & 7.9 & 69.5 & 10.9 & 89.0 & 5.2 & 95.4 & 3.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 4.2 & 0.9 & 4.1 & 1.2 & 4.0 & 1.5 & 3.0 & 0.8 & 2.9 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.1 & 0.2 & 2.1 & 0.6 & 4.1 & 1.5 & 6.0 & 1.7 & 11.9 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 6.1 & 2.1 & 7.2 & 2.9 & 7.0 & 1.6 & 6.7 & 0.7 & 6.0 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.5 & 0.5 & 3.7 & 1.5 & 7.1 & 1.6 & 13.7 & 1.4 & 24.4 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 19.9 & 5.3 & 18.6 & 1.5 & 17.0 & 0.9 & 16.8 & 0.6 & 15.2 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.1 & 1.3 & 9.5 & 0.7 & 17.3 & 0.9 & 34.3 & 1.0 & 61.9 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 29.7 & 3.7 & 29.5 & 2.2 & 31.2 & 1.7 & 31.8 & 1.6 & 21.4 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.6 & 0.9 & 15.0 & 1.0 & 31.8 & 1.6 & 64.9 & 3.2 & 87.3 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 48.0 & 2.0 & 51.5 & 1.7 & 55.7 & 1.4 & 44.6 & 0.6 & 23.6 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 12.2 & 0.6 & 26.2 & 1.0 & 56.7 & 1.3 & 90.8 & 1.2 & 96.2 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 71.9 & 3.1 & 75.6 & 3.3 & 76.9 & 2.3 & 46.5 & 0.5 & 24.1 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 18.3 & 0.9 & 38.5 & 1.8 & 78.4 & 2.4 & 94.7 & 1.0 & 98.1 & 0.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 88.2 & 3.3 & 89.8 & 1.3 & 81.5 & 1.6 & 47.2 & 0.6 & 24.3 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.5 & 0.8 & 45.7 & 0.7 & 83.1 & 1.4 & 96.0 & 0.9 & 98.9 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 94.4 & 1.6 & 93.5 & 1.0 & 80.0 & 2.3 & 47.0 & 0.7 & 24.3 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.0 & 0.5 & 47.6 & 0.7 & 81.5 & 2.2 & 95.8 & 1.1 & 98.8 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 97.4 & 0.2 & 95.1 & 0.8 & 81.2 & 2.2 & 47.5 & 0.8 & 24.3 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.8 & 0.2 & 48.4 & 0.5 & 82.7 & 2.2 & 96.7 & 1.4 & 98.8 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 98.4 & 1.0 & 96.1 & 1.0 & 81.7 & 2.0 & 47.5 & 0.5 & 24.3 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 0.3 & 49.0 & 0.6 & 83.2 & 2.1 & 96.7 & 0.7 & 99.0 & 0.2\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage

\begin{table}
    \centering
    \caption{twitch-ENGB (\lapgraph)}
    \label{tab:att_dp_twitch-ENGB-lap}    
    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.7 & 0.9 & 0.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.7 & 2.4 & 1.7 & 2.4\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 8.3 & 11.8 & 4.8 & 6.7 & 5.2 & 3.7 & 6.0 & 1.6 & 3.7 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.1 & 2.9 & 2.1 & 2.9 & 5.4 & 4.1 & 12.2 & 4.2 & 14.3 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 13.1 & 10.2 & 12.1 & 12.1 & 7.8 & 6.3 & 8.7 & 2.5 & 9.0 & 2.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.8 & 2.7 & 5.8 & 5.1 & 7.5 & 5.4 & 16.4 & 1.7 & 34.4 & 2.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 38.1 & 16.8 & 36.3 & 9.3 & 22.1 & 1.5 & 21.3 & 1.9 & 15.3 & 3.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 11.0 & 4.4 & 18.9 & 3.3 & 22.3 & 2.6 & 42.5 & 8.1 & 58.8 & 3.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 51.2 & 19.0 & 46.2 & 8.0 & 35.2 & 6.2 & 28.0 & 0.0 & 17.3 & 3.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.2 & 5.7 & 24.8 & 4.9 & 36.9 & 13.0 & 55.9 & 10.8 & 66.8 & 3.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 47.6 & 3.4 & 41.8 & 10.3 & 40.4 & 8.8 & 35.3 & 6.6 & 21.0 & 3.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 14.3 & 1.3 & 23.0 & 8.6 & 42.3 & 16.0 & 69.2 & 12.7 & 81.1 & 3.3\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.5 & 0.7 & 0.3 & 0.4 & 0.1 & 0.2 & 0.2 & 0.2 & 0.2 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.2 & 0.2 & 0.2 & 0.2 & 0.2 & 0.2 & 0.5 & 0.4 & 1.0 & 1.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 1.5 & 0.5 & 0.8 & 0.4 & 0.6 & 0.3 & 0.4 & 0.3 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.3 & 0.5 & 0.3 & 0.5 & 0.5 & 0.7 & 0.7 & 0.9 & 1.2 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 3.7 & 2.7 & 2.7 & 0.7 & 2.1 & 0.8 & 1.3 & 0.6 & 0.8 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.9 & 0.6 & 1.4 & 0.4 & 2.1 & 0.4 & 2.5 & 0.7 & 3.4 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 5.3 & 1.5 & 6.1 & 2.5 & 4.9 & 1.5 & 3.0 & 1.2 & 1.8 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 0.4 & 3.4 & 1.7 & 5.2 & 1.8 & 6.0 & 1.7 & 7.4 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 11.6 & 5.9 & 12.5 & 5.6 & 12.0 & 2.7 & 7.4 & 1.6 & 4.3 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.0 & 1.6 & 6.9 & 3.8 & 12.9 & 3.7 & 15.8 & 3.7 & 18.1 & 4.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 21.0 & 3.9 & 24.7 & 5.2 & 21.5 & 1.5 & 14.8 & 1.4 & 8.9 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.8 & 1.5 & 13.7 & 4.5 & 23.7 & 6.2 & 31.7 & 5.0 & 37.5 & 3.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 34.8 & 6.1 & 34.3 & 3.7 & 33.5 & 0.5 & 23.2 & 3.4 & 13.8 & 3.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.9 & 3.3 & 19.2 & 5.5 & 36.7 & 8.3 & 49.0 & 5.0 & 57.5 & 2.6\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 46.3 & 1.8 & 49.2 & 2.3 & 45.7 & 2.8 & 31.0 & 4.9 & 17.6 & 4.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.0 & 3.2 & 27.0 & 5.9 & 49.5 & 9.1 & 65.4 & 6.3 & 72.8 & 1.0\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 64.2 & 6.7 & 64.4 & 2.7 & 52.7 & 1.8 & 35.6 & 6.8 & 19.9 & 4.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.4 & 2.6 & 35.2 & 7.5 & 57.3 & 11.3 & 74.5 & 4.6 & 82.2 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 75.8 & 4.2 & 71.8 & 3.4 & 61.2 & 4.9 & 40.0 & 7.9 & 21.9 & 5.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.9 & 4.1 & 39.3 & 8.2 & 65.9 & 10.5 & 83.8 & 4.8 & 90.3 & 0.4\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 1.7 & 0.4 & 1.2 & 0.3 & 1.1 & 0.3 & 0.9 & 0.2 & 0.4 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.4 & 0.1 & 0.6 & 0.1 & 1.1 & 0.4 & 1.7 & 0.3 & 1.7 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 3.2 & 0.5 & 2.0 & 0.4 & 1.5 & 0.2 & 1.1 & 0.2 & 0.6 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.8 & 0.1 & 1.0 & 0.2 & 1.6 & 0.2 & 2.3 & 0.3 & 2.3 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 9.3 & 2.1 & 5.4 & 1.2 & 3.4 & 0.8 & 2.2 & 0.4 & 1.1 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.4 & 0.5 & 2.8 & 0.6 & 3.5 & 0.8 & 4.5 & 0.7 & 4.5 & 0.7\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 24.7 & 2.5 & 13.2 & 1.4 & 7.9 & 0.8 & 5.1 & 0.5 & 3.1 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.3 & 0.6 & 6.7 & 0.7 & 8.0 & 0.7 & 10.5 & 0.9 & 12.5 & 3.6\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 50.1 & 1.4 & 30.9 & 1.3 & 17.4 & 1.0 & 10.5 & 1.0 & 6.3 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 12.8 & 0.3 & 15.8 & 0.6 & 17.7 & 0.9 & 21.4 & 1.9 & 25.7 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 76.0 & 1.2 & 61.0 & 0.6 & 35.2 & 0.5 & 19.9 & 0.5 & 11.9 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.4 & 0.2 & 31.1 & 0.4 & 35.8 & 0.4 & 40.5 & 0.8 & 48.3 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 88.3 & 1.5 & 83.3 & 1.9 & 56.3 & 1.2 & 31.4 & 0.9 & 17.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.5 & 0.3 & 42.5 & 1.0 & 57.4 & 1.0 & 64.0 & 1.5 & 70.3 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 93.0 & 0.7 & 89.7 & 1.9 & 67.3 & 1.7 & 37.9 & 0.8 & 20.2 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.7 & 0.1 & 45.7 & 1.0 & 68.6 & 1.6 & 77.2 & 1.3 & 82.1 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 96.0 & 1.4 & 92.5 & 0.5 & 73.3 & 1.7 & 41.9 & 0.8 & 21.9 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.4 & 0.4 & 47.1 & 0.3 & 74.7 & 1.6 & 85.3 & 1.4 & 89.0 & 1.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 97.3 & 0.6 & 94.2 & 1.0 & 77.3 & 2.2 & 44.3 & 0.4 & 22.9 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.8 & 0.2 & 48.0 & 0.4 & 78.8 & 2.1 & 90.3 & 0.6 & 93.3 & 0.6\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{twitch-PTBR (\edgerand)}
    \label{tab:att_dp_twitch-PTBR-er}    

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.5 & 0.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & 0.9 & 1.3 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.5 & 0.2 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & 0.9 & 0.6 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 1.3 & 1.9 & 0.7 & 0.9 & 1.2 & 0.9 & 2.0 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.6 & 0.9 & 0.6 & 0.9 & 2.4 & 1.7 & 8.3 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 2.1 & 1.5 & 4.3 & 2.7 & 4.1 & 1.5 & 5.1 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 1.1 & 0.8 & 4.3 & 2.5 & 8.4 & 2.6 & 21.4 & 1.5\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 13.9 & 6.9 & 13.7 & 3.0 & 13.0 & 1.0 & 13.8 & 2.1 & 14.2 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.6 & 1.6 & 7.2 & 1.5 & 13.6 & 1.7 & 28.9 & 5.5 & 59.1 & 7.8\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 40.4 & 6.5 & 31.2 & 2.6 & 32.2 & 1.6 & 28.9 & 2.2 & 23.1 & 1.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.8 & 1.6 & 16.5 & 2.2 & 33.8 & 3.5 & 60.3 & 7.3 & 95.9 & 0.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 60.1 & 2.7 & 53.5 & 3.9 & 59.7 & 0.7 & 45.3 & 1.3 & 24.1 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.1 & 1.0 & 28.4 & 3.8 & 62.3 & 3.3 & 93.9 & 2.6 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 77.7 & 2.6 & 80.8 & 0.6 & 69.8 & 2.3 & 47.4 & 2.6 & 23.9 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.8 & 1.2 & 42.7 & 3.1 & 73.0 & 6.3 & 98.2 & 0.1 & 98.9 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 90.7 & 4.3 & 91.1 & 2.6 & 79.6 & 1.3 & 47.1 & 2.2 & 24.1 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.3 & 2.3 & 48.1 & 3.5 & 83.1 & 5.1 & 97.6 & 1.0 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 5.2 & 2.3 & 3.4 & 1.0 & 3.4 & 1.2 & 3.6 & 1.0 & 4.0 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 0.8 & 1.8 & 0.8 & 3.8 & 1.9 & 8.0 & 3.5 & 17.5 & 6.9\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 7.3 & 1.6 & 6.9 & 2.1 & 7.3 & 1.5 & 8.9 & 0.1 & 10.1 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.0 & 0.7 & 3.8 & 1.7 & 8.0 & 3.2 & 18.6 & 4.6 & 42.0 & 9.7\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 11.5 & 2.1 & 15.7 & 1.2 & 18.3 & 0.2 & 20.4 & 1.0 & 17.7 & 1.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.1 & 1.2 & 8.3 & 2.4 & 19.2 & 4.8 & 42.9 & 11.2 & 73.3 & 15.9\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 24.5 & 4.4 & 28.8 & 1.4 & 34.5 & 3.6 & 33.0 & 2.1 & 22.6 & 4.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.7 & 2.6 & 15.3 & 4.3 & 37.0 & 11.9 & 70.0 & 19.9 & 89.6 & 6.9\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 41.3 & 6.0 & 49.4 & 4.9 & 51.9 & 2.8 & 40.5 & 5.7 & 24.0 & 6.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 11.2 & 3.9 & 26.5 & 8.4 & 54.9 & 15.5 & 81.9 & 11.2 & 94.1 & 3.9\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 66.0 & 5.5 & 70.8 & 3.7 & 65.7 & 2.8 & 45.5 & 9.6 & 25.1 & 7.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.7 & 5.5 & 37.6 & 10.8 & 68.2 & 15.0 & 90.4 & 7.0 & 97.8 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 84.4 & 2.3 & 83.7 & 2.0 & 73.6 & 6.3 & 47.7 & 11.9 & 25.4 & 7.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.2 & 5.8 & 44.0 & 11.3 & 75.6 & 14.0 & 93.8 & 4.2 & 98.7 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 92.0 & 1.3 & 90.9 & 1.7 & 77.1 & 8.4 & 48.2 & 11.8 & 25.3 & 7.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.1 & 5.9 & 47.5 & 11.5 & 78.6 & 12.9 & 94.8 & 4.6 & 98.7 & 1.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 95.4 & 1.4 & 93.2 & 1.1 & 78.4 & 8.1 & 48.7 & 12.2 & 25.4 & 7.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 6.5 & 48.9 & 12.2 & 80.1 & 13.6 & 95.6 & 4.1 & 98.9 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.6 & 0.8 & 93.7 & 1.3 & 78.3 & 9.0 & 48.7 & 12.4 & 25.4 & 7.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 6.4 & 49.1 & 12.1 & 79.8 & 12.8 & 95.5 & 3.8 & 99.0 & 0.9\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 5.2 & 2.3 & 3.4 & 1.0 & 3.4 & 1.2 & 3.6 & 1.0 & 4.0 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 0.8 & 1.8 & 0.8 & 3.8 & 1.9 & 8.0 & 3.5 & 17.5 & 6.9\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 7.3 & 1.6 & 6.9 & 2.1 & 7.3 & 1.5 & 8.9 & 0.1 & 10.1 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.0 & 0.7 & 3.8 & 1.7 & 8.0 & 3.2 & 18.6 & 4.6 & 42.0 & 9.7\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 11.5 & 2.1 & 15.7 & 1.2 & 18.3 & 0.2 & 20.4 & 1.0 & 17.7 & 1.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.1 & 1.2 & 8.3 & 2.4 & 19.2 & 4.8 & 42.9 & 11.2 & 73.3 & 15.9\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 24.5 & 4.4 & 28.8 & 1.4 & 34.5 & 3.6 & 33.0 & 2.1 & 22.6 & 4.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.7 & 2.6 & 15.3 & 4.3 & 37.0 & 11.9 & 70.0 & 19.9 & 89.6 & 6.9\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 41.3 & 6.0 & 49.4 & 4.9 & 51.9 & 2.8 & 40.5 & 5.7 & 24.0 & 6.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 11.2 & 3.9 & 26.5 & 8.4 & 54.9 & 15.5 & 81.9 & 11.2 & 94.1 & 3.9\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 66.0 & 5.5 & 70.8 & 3.7 & 65.7 & 2.8 & 45.5 & 9.6 & 25.1 & 7.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.7 & 5.5 & 37.6 & 10.8 & 68.2 & 15.0 & 90.4 & 7.0 & 97.8 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 84.4 & 2.3 & 83.7 & 2.0 & 73.6 & 6.3 & 47.7 & 11.9 & 25.4 & 7.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.2 & 5.8 & 44.0 & 11.3 & 75.6 & 14.0 & 93.8 & 4.2 & 98.7 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 92.0 & 1.3 & 90.9 & 1.7 & 77.1 & 8.4 & 48.2 & 11.8 & 25.3 & 7.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.1 & 5.9 & 47.5 & 11.5 & 78.6 & 12.9 & 94.8 & 4.6 & 98.7 & 1.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 95.4 & 1.4 & 93.2 & 1.1 & 78.4 & 8.1 & 48.7 & 12.2 & 25.4 & 7.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 6.5 & 48.9 & 12.2 & 80.1 & 13.6 & 95.6 & 4.1 & 98.9 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.6 & 0.8 & 93.7 & 1.3 & 78.3 & 9.0 & 48.7 & 12.4 & 25.4 & 7.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 6.4 & 49.1 & 12.1 & 79.8 & 12.8 & 95.5 & 3.8 & 99.0 & 0.9\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage

\begin{table}
    \centering
    \caption{twitch-PTBR (\lapgraph)}
    \label{tab:att_dp_twitch-PTBR-lap}    
    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 0.4 & 0.5 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 0.8 & 2.3 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 2.1 & 2.9 & 1.0 & 1.5 & 2.3 & 0.7 & 2.7 & 1.0 & 1.8 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.6 & 0.8 & 0.6 & 0.8 & 2.4 & 0.8 & 5.4 & 1.8 & 7.2 & 1.8\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 4.6 & 3.3 & 3.4 & 2.6 & 2.4 & 1.7 & 4.0 & 0.7 & 4.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.2 & 0.9 & 1.8 & 1.4 & 2.5 & 1.7 & 8.3 & 1.6 & 17.9 & 2.4\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 6.7 & 0.7 & 6.8 & 0.8 & 10.2 & 0.7 & 10.2 & 0.9 & 8.9 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.8 & 0.1 & 3.6 & 0.2 & 10.7 & 0.9 & 21.3 & 3.0 & 36.8 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 22.8 & 5.7 & 17.1 & 2.1 & 15.0 & 2.2 & 14.4 & 1.7 & 13.9 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.0 & 1.2 & 9.0 & 0.5 & 15.5 & 1.4 & 30.1 & 5.1 & 58.1 & 6.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 27.4 & 8.2 & 24.2 & 5.7 & 23.3 & 2.0 & 22.5 & 3.9 & 19.7 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.2 & 1.9 & 12.6 & 2.1 & 24.4 & 2.6 & 47.1 & 10.2 & 82.2 & 10.5\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 22.3 & 2.6 & 27.0 & 1.4 & 27.2 & 2.1 & 30.1 & 1.5 & 21.9 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.9 & 0.6 & 14.3 & 0.7 & 28.4 & 3.0 & 62.8 & 6.4 & 90.9 & 4.5\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 40.9 & 9.5 & 39.7 & 3.1 & 39.0 & 2.9 & 39.3 & 1.9 & 23.1 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.8 & 2.0 & 20.8 & 0.4 & 40.8 & 4.6 & 81.8 & 7.5 & 95.7 & 2.5\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 6.1 & 0.8 & 5.0 & 0.3 & 4.2 & 0.4 & 3.6 & 0.6 & 2.9 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.6 & 0.3 & 2.6 & 0.6 & 4.4 & 1.0 & 7.4 & 1.1 & 12.1 & 2.7\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 12.0 & 1.8 & 11.0 & 0.9 & 9.6 & 0.7 & 7.2 & 1.2 & 4.8 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.1 & 0.6 & 5.6 & 1.1 & 10.1 & 2.6 & 14.4 & 1.9 & 19.6 & 3.2\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 18.6 & 1.3 & 19.8 & 1.1 & 19.8 & 1.2 & 14.1 & 3.3 & 8.5 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.8 & 1.1 & 10.5 & 2.9 & 20.8 & 5.2 & 27.9 & 1.9 & 33.8 & 3.5\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 25.0 & 1.8 & 33.2 & 3.8 & 33.8 & 2.9 & 23.9 & 5.5 & 13.7 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.7 & 2.0 & 17.9 & 5.9 & 35.6 & 9.7 & 47.3 & 3.0 & 54.1 & 3.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 41.3 & 0.9 & 49.7 & 4.2 & 47.9 & 2.8 & 32.8 & 6.8 & 18.5 & 4.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.9 & 2.9 & 26.5 & 8.1 & 49.7 & 10.8 & 65.3 & 5.2 & 73.0 & 3.8\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 55.2 & 6.3 & 62.6 & 4.0 & 58.6 & 4.0 & 39.0 & 9.0 & 21.7 & 5.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 14.9 & 4.9 & 33.3 & 9.7 & 60.5 & 12.3 & 77.0 & 4.7 & 84.9 & 2.8\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 66.6 & 6.5 & 71.8 & 5.1 & 66.0 & 5.1 & 42.8 & 10.3 & 23.1 & 6.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.8 & 5.6 & 38.2 & 11.1 & 67.9 & 13.1 & 84.4 & 4.4 & 90.4 & 2.4\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 75.1 & 4.9 & 78.0 & 3.4 & 68.6 & 5.1 & 44.6 & 10.5 & 24.0 & 6.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.0 & 5.8 & 41.2 & 11.0 & 70.7 & 14.0 & 88.1 & 5.1 & 93.9 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 81.5 & 5.5 & 84.1 & 3.3 & 73.2 & 5.7 & 46.0 & 10.4 & 24.7 & 6.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.7 & 6.5 & 44.5 & 12.2 & 75.3 & 14.3 & 90.9 & 5.8 & 96.2 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 87.2 & 2.2 & 88.2 & 1.5 & 75.8 & 7.4 & 47.1 & 11.5 & 24.9 & 7.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.0 & 6.1 & 46.4 & 12.0 & 77.6 & 13.6 & 92.7 & 4.6 & 96.9 & 1.6\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 10.3 & 0.9 & 9.1 & 0.1 & 8.3 & 0.5 & 6.8 & 0.4 & 5.4 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.5 & 0.2 & 4.5 & 0.6 & 8.1 & 0.7 & 13.3 & 1.3 & 21.0 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 21.8 & 1.4 & 19.9 & 0.8 & 14.7 & 0.7 & 10.4 & 0.5 & 7.6 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.4 & 0.4 & 9.8 & 0.9 & 14.5 & 1.0 & 20.4 & 1.7 & 29.7 & 3.3\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 40.2 & 2.8 & 37.8 & 2.2 & 28.7 & 2.1 & 18.0 & 1.5 & 11.3 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.8 & 0.6 & 18.5 & 1.5 & 28.0 & 1.3 & 35.2 & 1.2 & 44.3 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 53.9 & 1.3 & 58.4 & 1.5 & 48.4 & 4.9 & 28.2 & 2.8 & 16.3 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.2 & 1.2 & 28.7 & 2.8 & 47.2 & 1.0 & 54.9 & 1.3 & 63.7 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 70.0 & 0.6 & 73.2 & 1.4 & 64.0 & 5.2 & 37.3 & 3.7 & 20.5 & 2.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.2 & 1.8 & 36.0 & 3.6 & 62.5 & 2.1 & 72.7 & 1.3 & 79.9 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 79.9 & 1.1 & 82.0 & 1.7 & 74.2 & 5.7 & 42.9 & 4.3 & 22.9 & 2.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.7 & 2.2 & 40.4 & 3.9 & 72.5 & 2.7 & 83.6 & 1.0 & 89.2 & 0.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 86.8 & 0.7 & 89.1 & 0.7 & 80.0 & 5.9 & 46.0 & 5.0 & 24.0 & 2.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.4 & 2.3 & 43.9 & 4.8 & 78.2 & 3.3 & 89.6 & 0.3 & 93.7 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 89.8 & 1.5 & 90.6 & 2.1 & 79.5 & 5.4 & 47.5 & 5.0 & 24.6 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 22.1 & 2.3 & 44.6 & 4.1 & 77.8 & 3.6 & 92.5 & 0.6 & 95.9 & 0.4\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 93.5 & 1.3 & 94.4 & 1.2 & 83.5 & 5.9 & 48.5 & 5.1 & 25.0 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.0 & 2.3 & 46.5 & 4.7 & 81.6 & 3.7 & 94.6 & 0.7 & 97.3 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.4 & 0.9 & 95.8 & 1.0 & 85.5 & 6.3 & 49.5 & 5.3 & 25.2 & 2.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.5 & 2.5 & 47.2 & 4.9 & 83.6 & 3.7 & 96.4 & 0.4 & 98.3 & 0.1\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{PPI (\edgerand)}
    \label{tab:att_dp_twitch-PTBR-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 3.7 & 2.8\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 2.7 & 3.8 & 3.3 & 2.5 & 4.3 & 3.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 2.8 & 3.9 & 6.2 & 4.5 & 16.4 & 11.6\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 4.8 & 6.7 & 5.1 & 3.6 & 7.9 & 3.3 & 14.7 & 7.5 & 15.3 & 6.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 2.0 & 2.5 & 1.8 & 7.4 & 3.8 & 27.5 & 15.3 & 57.0 & 27.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 14.3 & 11.7 & 24.9 & 6.8 & 26.4 & 4.0 & 32.7 & 7.4 & 27.7 & 2.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.9 & 3.4 & 12.0 & 4.0 & 24.3 & 6.5 & 60.1 & 20.7 & 97.9 & 2.9\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 51.2 & 19.4 & 55.3 & 15.3 & 54.1 & 7.4 & 52.7 & 4.1 & 28.3 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.4 & 5.1 & 26.1 & 6.5 & 48.9 & 8.1 & 93.8 & 8.8 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 59.5 & 8.9 & 77.7 & 5.4 & 78.9 & 4.1 & 56.7 & 6.6 & 28.3 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.7 & 3.7 & 37.2 & 6.3 & 71.1 & 5.8 & 100.0 & 0.0 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}
\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.5 & 0.8 & 0.4 & 0.3 & 0.5 & 0.2 & 0.6 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.2 & 0.3 & 0.4 & 0.3 & 1.1 & 0.5 & 2.5 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 1.6 & 2.2 & 1.6 & 1.1 & 1.6 & 0.7 & 1.6 & 0.7 & 1.1 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.5 & 0.7 & 0.9 & 0.7 & 1.7 & 0.8 & 3.4 & 2.0 & 4.7 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 3.7 & 2.0 & 4.5 & 1.6 & 4.0 & 1.6 & 3.3 & 1.1 & 3.2 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.0 & 0.6 & 2.4 & 1.1 & 4.3 & 2.1 & 6.7 & 2.2 & 12.8 & 1.7\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 8.5 & 2.0 & 6.4 & 2.6 & 6.9 & 1.5 & 7.4 & 1.3 & 6.6 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.3 & 0.8 & 3.4 & 1.7 & 7.2 & 1.7 & 15.1 & 1.8 & 26.7 & 3.3\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 9.5 & 3.4 & 12.3 & 2.3 & 12.5 & 3.0 & 12.5 & 2.1 & 19.1 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.6 & 1.2 & 6.4 & 1.8 & 12.8 & 2.4 & 25.5 & 3.0 & 78.4 & 4.5\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 20.1 & 5.8 & 20.8 & 6.0 & 24.9 & 1.6 & 41.5 & 2.8 & 24.4 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.2 & 1.4 & 10.6 & 2.4 & 25.8 & 2.9 & 85.7 & 9.9 & 99.7 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 33.3 & 5.6 & 42.9 & 5.1 & 59.7 & 3.9 & 48.8 & 5.5 & 24.4 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.5 & 0.7 & 21.9 & 0.7 & 61.5 & 3.8 & 99.7 & 0.2 & 99.7 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 54.5 & 6.5 & 70.1 & 4.0 & 78.0 & 2.8 & 48.8 & 5.5 & 24.4 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 14.3 & 3.0 & 36.4 & 5.4 & 80.5 & 6.9 & 99.7 & 0.2 & 99.7 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 82.5 & 3.4 & 88.3 & 0.4 & 85.7 & 4.4 & 49.0 & 5.4 & 24.5 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.6 & 3.2 & 45.7 & 5.1 & 88.3 & 5.4 & 100.0 & 0.0 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 90.5 & 2.2 & 93.3 & 1.0 & 87.9 & 5.6 & 49.0 & 5.4 & 24.5 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.7 & 3.2 & 48.4 & 5.7 & 90.4 & 4.3 & 100.0 & 0.0 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 2.5 & 1.1 & 2.2 & 0.6 & 2.6 & 0.2 & 3.0 & 0.2 & 3.2 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.5 & 0.2 & 0.9 & 0.3 & 2.3 & 0.1 & 5.2 & 0.2 & 11.1 & 0.7\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 8.0 & 2.0 & 8.5 & 1.7 & 8.1 & 1.0 & 8.1 & 0.6 & 7.9 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.7 & 0.4 & 3.7 & 0.6 & 7.0 & 0.6 & 14.0 & 0.5 & 27.4 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 19.2 & 3.3 & 19.6 & 0.9 & 18.9 & 1.1 & 18.0 & 1.2 & 18.0 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.2 & 0.6 & 8.5 & 0.2 & 16.3 & 0.6 & 31.1 & 1.0 & 62.3 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 38.9 & 1.7 & 38.8 & 1.6 & 36.6 & 1.4 & 35.5 & 0.8 & 28.3 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.4 & 0.3 & 16.8 & 0.4 & 31.8 & 0.6 & 61.6 & 1.5 & 98.3 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 59.8 & 1.8 & 58.1 & 0.9 & 58.6 & 0.4 & 57.3 & 2.3 & 28.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.0 & 0.5 & 25.2 & 0.7 & 50.9 & 1.7 & 99.4 & 0.1 & 99.6 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 77.1 & 2.1 & 77.3 & 1.5 & 79.4 & 1.3 & 57.6 & 2.4 & 28.8 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.7 & 0.7 & 33.6 & 1.4 & 69.0 & 2.2 & 99.9 & 0.1 & 99.9 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 89.3 & 2.4 & 90.0 & 1.2 & 91.6 & 1.2 & 57.7 & 2.3 & 28.8 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.4 & 0.7 & 39.1 & 1.4 & 79.6 & 3.1 & 100.0 & 0.0 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 95.4 & 1.3 & 96.0 & 1.0 & 95.7 & 0.7 & 57.7 & 2.3 & 28.8 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.7 & 0.7 & 41.7 & 1.4 & 83.1 & 3.1 & 100.0 & 0.0 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 97.2 & 0.4 & 97.9 & 0.3 & 97.0 & 0.2 & 57.7 & 2.3 & 28.8 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.1 & 0.9 & 42.5 & 1.8 & 84.3 & 3.4 & 100.0 & 0.0 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 99.0 & 0.5 & 99.1 & 0.1 & 97.6 & 0.2 & 57.7 & 2.3 & 28.8 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.5 & 0.8 & 43.1 & 1.7 & 84.8 & 3.2 & 100.0 & 0.0 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{PPI (\lapgraph)}
    \label{tab:att_dp_twitch-PTBR-lap}    
    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.7 & 0.9 & 1.3 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 1.6 & 4.8 & 4.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 1.3 & 1.9 & 4.0 & 1.6 & 5.0 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 & 1.6 & 6.9 & 2.6 & 18.0 & 3.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 5.1 & 3.6 & 6.7 & 6.8 & 8.0 & 3.3 & 13.0 & 4.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 2.5 & 1.8 & 6.0 & 5.8 & 14.5 & 6.1 & 46.8 & 16.7\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 4.8 & 6.7 & 15.4 & 12.6 & 14.7 & 13.2 & 18.0 & 7.1 & 19.0 & 5.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 2.0 & 7.4 & 5.7 & 13.4 & 11.3 & 33.2 & 14.8 & 68.8 & 22.5\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 4.8 & 6.7 & 12.8 & 9.6 & 21.3 & 15.4 & 29.3 & 12.3 & 23.7 & 2.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 2.0 & 6.2 & 4.5 & 20.1 & 14.2 & 54.5 & 25.9 & 84.5 & 11.2\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 17.9 & 5.1 & 32.6 & 4.2 & 39.7 & 11.7 & 42.7 & 8.2 & 27.0 & 4.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.6 & 1.2 & 15.5 & 2.1 & 36.7 & 13.2 & 77.1 & 19.2 & 94.9 & 3.6\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 0.7 & 0.5 & 0.4 & 0.7 & 0.2 & 0.5 & 0.1 & 0.5 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.3 & 0.2 & 0.3 & 0.2 & 0.7 & 0.1 & 0.9 & 0.1 & 2.0 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 2.6 & 2.7 & 1.6 & 1.3 & 1.9 & 1.1 & 1.1 & 0.5 & 0.6 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.6 & 0.6 & 0.8 & 0.6 & 1.8 & 1.1 & 2.2 & 1.0 & 2.5 & 1.1\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 2.6 & 1.5 & 2.9 & 1.0 & 3.7 & 1.8 & 2.5 & 1.1 & 1.2 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.7 & 0.3 & 1.5 & 0.4 & 3.8 & 1.8 & 4.9 & 2.2 & 4.9 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 7.9 & 3.9 & 6.7 & 2.6 & 9.7 & 2.4 & 5.8 & 1.7 & 3.0 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.0 & 0.8 & 3.3 & 1.0 & 9.8 & 1.6 & 11.7 & 2.9 & 12.1 & 2.9\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 10.1 & 1.5 & 14.1 & 3.3 & 20.4 & 3.5 & 12.4 & 1.7 & 6.5 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.6 & 0.5 & 7.2 & 1.4 & 20.9 & 2.6 & 25.2 & 2.1 & 26.6 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 19.0 & 0.0 & 24.0 & 3.5 & 38.3 & 4.7 & 23.3 & 3.7 & 12.3 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.0 & 0.6 & 12.5 & 2.7 & 39.3 & 3.4 & 47.4 & 3.0 & 49.9 & 4.5\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 30.2 & 5.6 & 42.4 & 8.5 & 56.9 & 4.7 & 33.0 & 4.9 & 17.3 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.0 & 2.4 & 22.2 & 6.5 & 58.5 & 2.2 & 67.1 & 2.9 & 70.1 & 3.5\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 49.2 & 5.9 & 61.9 & 5.9 & 69.3 & 5.4 & 39.1 & 5.1 & 19.9 & 2.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.0 & 2.9 & 32.1 & 4.9 & 71.2 & 2.4 & 79.8 & 1.8 & 81.2 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 63.5 & 7.2 & 74.4 & 4.1 & 76.1 & 5.5 & 43.4 & 5.9 & 22.2 & 3.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.7 & 3.6 & 38.5 & 4.6 & 78.2 & 3.1 & 88.4 & 2.3 & 90.6 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 79.9 & 3.0 & 84.8 & 1.7 & 81.5 & 5.1 & 45.5 & 5.6 & 23.1 & 2.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.9 & 3.1 & 43.9 & 5.0 & 83.8 & 4.3 & 92.8 & 1.3 & 94.3 & 1.3\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 2.4 & 0.5 & 2.0 & 0.5 & 1.5 & 0.4 & 1.4 & 0.1 & 1.3 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.5 & 0.1 & 0.9 & 0.2 & 1.3 & 0.3 & 2.5 & 0.1 & 4.6 & 0.2\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 6.3 & 1.5 & 3.8 & 0.9 & 2.6 & 0.5 & 1.8 & 0.3 & 1.6 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 0.3 & 1.6 & 0.4 & 2.2 & 0.4 & 3.1 & 0.5 & 5.7 & 0.7\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 17.0 & 3.4 & 9.1 & 1.8 & 5.5 & 0.9 & 3.6 & 0.6 & 2.5 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.7 & 0.6 & 3.9 & 0.7 & 4.7 & 0.6 & 6.1 & 0.8 & 8.6 & 1.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 35.9 & 3.2 & 23.5 & 2.3 & 13.1 & 1.5 & 7.6 & 0.7 & 5.0 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.8 & 0.5 & 10.2 & 0.7 & 11.3 & 0.8 & 13.2 & 0.8 & 17.1 & 1.6\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 56.8 & 0.4 & 53.5 & 2.8 & 29.1 & 1.7 & 17.1 & 0.8 & 10.7 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 12.3 & 0.4 & 23.2 & 0.3 & 25.3 & 0.6 & 29.7 & 0.5 & 37.2 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 74.8 & 0.3 & 79.2 & 0.9 & 55.8 & 1.7 & 31.7 & 0.9 & 18.3 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.2 & 0.6 & 34.4 & 1.5 & 48.4 & 0.6 & 54.9 & 0.8 & 63.4 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 86.6 & 1.2 & 88.8 & 0.4 & 79.8 & 3.8 & 43.1 & 2.2 & 23.4 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 18.8 & 1.0 & 38.6 & 1.6 & 69.2 & 1.0 & 74.7 & 1.1 & 81.0 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 92.5 & 1.1 & 93.2 & 0.8 & 90.1 & 2.3 & 49.1 & 2.3 & 26.0 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.1 & 1.0 & 40.5 & 1.6 & 78.2 & 1.5 & 85.2 & 0.7 & 90.0 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 95.9 & 0.7 & 96.4 & 0.5 & 94.3 & 0.7 & 52.8 & 2.4 & 27.3 & 1.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 20.8 & 0.9 & 41.9 & 1.8 & 81.9 & 2.8 & 91.5 & 0.6 & 94.7 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 97.4 & 0.3 & 97.8 & 0.3 & 95.5 & 0.2 & 54.6 & 2.2 & 27.8 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 21.2 & 0.8 & 42.5 & 1.8 & 82.9 & 3.1 & 94.6 & 0.2 & 96.5 & 0.2\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{Flickr (\edgerand)}
    \label{tab:att_dp_twitch-PTBR-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.6 & 3.6 & 1.3 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 5.6 & 7.9 & 5.6 & 7.9\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 16.7 & 23.6 & 8.3 & 11.8 & 4.8 & 6.7 & 2.6 & 3.6 & 1.3 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.6 & 7.9 & 5.6 & 7.9 & 5.6 & 7.9 & 5.6 & 7.9 & 5.6 & 7.9\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 16.7 & 23.6 & 8.3 & 11.8 & 4.8 & 6.7 & 8.5 & 6.4 & 4.3 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.6 & 7.9 & 5.6 & 7.9 & 5.6 & 7.9 & 17.8 & 13.7 & 17.8 & 13.7\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 33.3 & 47.1 & 16.7 & 23.6 & 28.1 & 15.7 & 20.1 & 3.9 & 10.4 & 2.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.3 & 11.8 & 8.3 & 11.8 & 28.9 & 15.0 & 41.1 & 6.8 & 41.1 & 6.8\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 66.7 & 47.1 & 38.9 & 28.3 & 37.9 & 15.7 & 19.3 & 7.7 & 12.9 & 5.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 24.4 & 17.5 & 24.4 & 17.5 & 39.4 & 14.9 & 39.4 & 14.9 & 51.7 & 22.5\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.3 & 1.9 & 0.7 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 3.1 & 2.2 & 3.1\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 2.6 & 3.6 & 2.7 & 1.9 & 1.3 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 2.4 & 3.4 & 4.6 & 3.3 & 4.6 & 3.3\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 4.8 & 6.7 & 2.6 & 3.6 & 4.0 & 5.7 & 3.5 & 1.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 2.4 & 3.4 & 2.4 & 3.4 & 7.1 & 10.1 & 12.7 & 6.3\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 8.3 & 11.8 & 9.5 & 6.7 & 13.6 & 2.5 & 11.3 & 0.9 & 7.2 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.2 & 3.1 & 4.6 & 3.3 & 12.5 & 1.8 & 20.5 & 0.7 & 26.2 & 4.4\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 27.8 & 3.9 & 21.0 & 5.9 & 17.7 & 9.3 & 18.0 & 10.7 & 11.0 & 3.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.9 & 1.5 & 10.3 & 3.1 & 17.0 & 9.7 & 34.1 & 21.8 & 41.0 & 16.4\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 14.9 & 4.9 & 9.8 & 3.2 & 6.1 & 1.8 & 4.1 & 0.6 & 2.6 & 0.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.9 & 1.6 & 5.1 & 2.1 & 6.3 & 2.4 & 8.2 & 2.0 & 10.6 & 2.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 32.4 & 4.2 & 26.8 & 3.3 & 16.8 & 2.1 & 11.0 & 1.4 & 7.2 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.2 & 1.7 & 13.6 & 3.0 & 17.1 & 3.8 & 22.2 & 5.1 & 29.1 & 4.7\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 38.1 & 1.7 & 34.7 & 2.6 & 23.3 & 3.7 & 15.7 & 1.8 & 9.9 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.6 & 1.4 & 17.6 & 3.0 & 23.7 & 5.9 & 31.5 & 5.7 & 39.8 & 6.4\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 34.5 & 3.1 & 35.2 & 2.9 & 25.6 & 2.8 & 16.5 & 1.9 & 10.5 & 0.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 8.8 & 1.7 & 17.9 & 3.3 & 25.8 & 4.7 & 33.4 & 6.4 & 42.3 & 5.5\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 24.6 & 3.8 & 32.0 & 5.4 & 24.2 & 2.9 & 14.9 & 1.4 & 9.7 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.3 & 1.6 & 16.4 & 4.4 & 24.5 & 5.0 & 30.0 & 5.3 & 38.9 & 5.3\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 19.6 & 4.2 & 25.3 & 6.2 & 20.6 & 3.1 & 14.4 & 2.1 & 9.7 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.0 & 1.5 & 13.0 & 4.4 & 20.9 & 5.0 & 29.0 & 6.5 & 39.1 & 7.5\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage


\begin{table}
    \centering
    \caption{Flickr (\lapgraph)}
    \label{tab:att_dp_twitch-PTBR-lap}    
    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 6.7 & 9.4 & 3.3 & 4.7 & 6.1 & 5.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 6.7 & 9.4 & 6.7 & 9.4 & 23.3 & 20.5\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 11.1 & 15.7 & 26.4 & 10.5 & 13.4 & 5.1 & 6.9 & 2.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 6.7 & 9.4 & 27.2 & 9.7 & 27.2 & 9.7 & 27.2 & 9.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 11.1 & 15.7 & 16.2 & 12.0 & 21.9 & 7.2 & 14.8 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 6.7 & 9.4 & 17.8 & 13.7 & 45.0 & 14.7 & 58.9 & 6.8\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 4.8 & 6.7 & 2.6 & 3.6 & 1.3 & 1.9 & 0.7 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 2.2 & 3.1 & 2.2 & 3.1 & 2.2 & 3.1 & 2.2 & 3.1\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 2.6 & 3.6 & 1.3 & 1.9 & 1.3 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 3.1 & 2.2 & 3.1 & 4.6 & 3.3\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 4.8 & 6.7 & 2.6 & 3.6 & 1.3 & 1.9 & 1.3 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 2.2 & 3.1 & 2.2 & 3.1 & 2.2 & 3.1 & 4.6 & 3.3\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 2.6 & 3.6 & 4.0 & 3.3 & 2.0 & 1.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 3.1 & 6.8 & 5.4 & 6.8 & 5.4\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 2.6 & 3.6 & 5.3 & 5.0 & 3.3 & 2.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 3.1 & 9.0 & 8.3 & 11.4 & 8.4\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 8.3 & 11.8 & 4.8 & 6.7 & 2.6 & 3.6 & 5.3 & 5.0 & 4.0 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.2 & 3.1 & 2.2 & 3.1 & 2.2 & 3.1 & 9.4 & 9.0 & 14.0 & 11.7\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 19.4 & 14.2 & 16.2 & 12.0 & 14.4 & 5.1 & 10.0 & 1.6 & 7.0 & 3.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.6 & 4.2 & 7.8 & 5.7 & 13.5 & 5.3 & 18.3 & 3.5 & 25.4 & 12.6\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering\vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.4 & 0.5 & 0.2 & 0.3 & 0.1 & 0.1 & 0.0 & 0.1 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.4 & 0.5 & 0.2 & 0.3 & 0.1 & 0.1 & 0.0 & 0.1 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.4 & 0.5 & 0.2 & 0.3 & 0.1 & 0.1 & 0.0 & 0.1 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 1.6 & 1.3 & 1.0 & 0.9 & 0.6 & 0.5 & 0.3 & 0.2 & 0.2 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.4 & 0.4 & 0.5 & 0.5 & 0.6 & 0.5 & 0.6 & 0.5 & 0.6 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 3.5 & 1.3 & 2.0 & 0.9 & 1.2 & 0.5 & 0.6 & 0.3 & 0.3 & 0.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.9 & 0.4 & 1.0 & 0.5 & 1.2 & 0.5 & 1.2 & 0.5 & 1.2 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 11.5 & 0.9 & 7.9 & 0.5 & 5.0 & 0.7 & 2.5 & 0.4 & 1.3 & 0.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.9 & 0.5 & 4.0 & 0.7 & 5.0 & 0.3 & 5.0 & 0.3 & 5.0 & 0.3\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 18.2 & 2.2 & 14.8 & 0.7 & 11.4 & 1.4 & 7.6 & 1.2 & 3.9 & 0.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.6 & 0.9 & 7.4 & 0.8 & 11.6 & 2.5 & 15.0 & 1.2 & 15.2 & 1.3\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 19.6 & 0.7 & 16.9 & 0.6 & 14.1 & 1.1 & 11.9 & 0.8 & 9.0 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.9 & 0.4 & 8.5 & 1.3 & 14.2 & 2.2 & 24.0 & 3.3 & 35.7 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 15.9 & 1.7 & 17.8 & 3.2 & 15.6 & 1.7 & 12.9 & 1.3 & 10.6 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.0 & 0.7 & 9.1 & 2.5 & 15.9 & 3.4 & 26.2 & 5.4 & 43.1 & 8.5\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 14.5 & 3.3 & 19.7 & 3.7 & 16.9 & 2.1 & 13.1 & 1.4 & 10.8 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 3.7 & 1.1 & 10.0 & 2.5 & 17.1 & 3.4 & 26.5 & 5.5 & 43.6 & 8.1\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}
\newpage

}




==> tables/tab_attack_dp_selected.tex <==
{

\setlength{\tabcolsep}{4pt} % column sep

\begin{table}
    \centering
    \caption{twitch-RU (\edgerand)}
    \label{tab:att_dp_twitch-RU-er}    
    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{low}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 0.0 & 0.0 & 0.0 & 0.0 & 1.3 & 1.9 & 1.3 & 1.9 & 1.3 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.0 & 0.0 & 0.0 & 0.0 & 1.5 & 2.1 & 3.0 & 4.3 & 6.2 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 4.8 & 6.7 & 5.1 & 7.3 & 4.0 & 3.3 & 3.3 & 1.9 & 2.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.5 & 2.1 & 3.0 & 4.3 & 4.8 & 3.7 & 7.7 & 4.2 & 12.8 & 6.0\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 19.0 & 6.7 & 12.8 & 3.6 & 9.3 & 1.9 & 8.0 & 2.8 & 6.7 & 3.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.2 & 2.1 & 7.7 & 1.7 & 11.0 & 2.0 & 18.7 & 6.2 & 31.5 & 15.1\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 28.6 & 11.7 & 25.6 & 13.1 & 17.3 & 10.0 & 16.7 & 4.7 & 16.7 & 2.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 9.5 & 3.9 & 16.0 & 8.3 & 20.8 & 11.9 & 39.9 & 13.2 & 78.9 & 12.8\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 38.1 & 17.8 & 38.5 & 10.9 & 38.7 & 7.5 & 34.0 & 1.6 & 20.7 & 1.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 12.8 & 6.0 & 24.0 & 7.9 & 46.1 & 11.5 & 80.3 & 8.2 & 97.0 & 2.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 71.4 & 11.7 & 56.4 & 3.6 & 57.3 & 5.0 & 39.3 & 1.9 & 21.3 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.7 & 4.4 & 34.5 & 2.1 & 67.4 & 6.1 & 92.7 & 7.4 & 100.0 & 0.0\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 95.2 & 6.7 & 79.5 & 3.6 & 73.3 & 1.9 & 42.0 & 3.3 & 21.3 & 1.7\\
& \multicolumn{1}{c}{\scriptsize recall} & 31.5 & 4.0 & 48.6 & 3.0 & 86.4 & 5.9 & 98.5 & 2.1 & 100.0 & 0.0\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{unconstrained}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 0.7 & 0.1 & 0.6 & 0.1 & 1.2 & 0.4 & 1.6 & 0.6 & 1.5 & 0.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.2 & 0.0 & 0.3 & 0.1 & 1.3 & 0.4 & 3.4 & 1.3 & 6.4 & 1.9\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 1.1 & 1.5 & 2.1 & 1.3 & 2.3 & 1.2 & 2.1 & 0.7 & 2.1 & 0.6\\
& \multicolumn{1}{c}{\scriptsize recall} & 0.3 & 0.4 & 1.2 & 0.7 & 2.5 & 1.3 & 4.5 & 1.6 & 9.2 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 5.2 & 4.3 & 5.8 & 2.6 & 7.2 & 1.8 & 6.4 & 1.7 & 6.4 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.4 & 1.1 & 3.1 & 1.3 & 7.8 & 1.7 & 13.8 & 3.1 & 27.8 & 5.3\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 5.5 & 2.7 & 7.5 & 2.2 & 9.0 & 2.0 & 11.6 & 2.0 & 15.4 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 1.5 & 0.7 & 4.0 & 1.0 & 9.7 & 1.7 & 25.2 & 3.6 & 66.9 & 7.4\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 9.2 & 3.9 & 12.4 & 3.1 & 21.1 & 3.2 & 30.9 & 3.6 & 20.3 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.5 & 1.0 & 6.7 & 1.4 & 22.9 & 2.8 & 67.2 & 5.3 & 88.6 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 22.1 & 4.5 & 36.2 & 4.4 & 45.1 & 2.8 & 36.5 & 1.5 & 21.2 & 0.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 6.0 & 0.9 & 19.7 & 1.6 & 49.2 & 1.0 & 79.7 & 1.6 & 92.5 & 1.0\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 55.1 & 2.4 & 61.9 & 2.9 & 55.7 & 3.2 & 39.8 & 1.5 & 22.3 & 0.8\\
& \multicolumn{1}{c}{\scriptsize recall} & 15.0 & 0.4 & 33.8 & 0.4 & 60.8 & 1.5 & 86.8 & 0.6 & 97.1 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 72.1 & 6.4 & 75.6 & 5.0 & 66.5 & 3.1 & 43.2 & 1.9 & 22.5 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 19.7 & 1.2 & 41.3 & 1.5 & 72.6 & 1.2 & 94.2 & 0.2 & 98.3 & 0.1\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 87.5 & 1.9 & 85.9 & 1.7 & 70.5 & 2.2 & 43.5 & 1.7 & 22.5 & 1.0\\
& \multicolumn{1}{c}{\scriptsize recall} & 23.9 & 0.8 & 47.0 & 1.1 & 77.0 & 2.2 & 94.9 & 1.4 & 98.2 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 91.9 & 3.3 & 86.9 & 0.9 & 70.8 & 2.3 & 43.0 & 2.0 & 22.5 & 1.1\\
& \multicolumn{1}{c}{\scriptsize recall} & 25.1 & 1.2 & 47.5 & 1.6 & 77.3 & 2.0 & 93.7 & 1.5 & 98.0 & 0.7\\
\bottomrule
    \end{tabular}%
}

\end{subtable}

    \begin{subtable}[]{\linewidth}
    \centering     \vspace{0.5em}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{cc
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
  >{\collectcell\num}R{2.18em}<{\endcollectcell}
  @{\tiny${}\pm{}$}
  >{\tiny\collectcell\num}R{1.308em}<{\endcollectcell}
}
    \toprule
    % \multirow{2}{*}{ratio}     
\multicolumn{2}{c}{\footnotesize \textbf{high}}&  \multicolumn{2}{c}{\scriptsize $\hat k=k/4$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k/2$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=2k$}  
    &  \multicolumn{2}{c}{\scriptsize $\hat k=4k$}  \\\midrule
\multirow{2}{*}{$\varepsilon=1$} & \multicolumn{1}{c}{\scriptsize precision} & 15.6 & 9.1 & 11.2 & 4.6 & 9.2 & 3.7 & 7.1 & 2.5 & 5.5 & 1.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 2.8 & 1.4 & 4.0 & 1.4 & 6.6 & 2.2 & 10.2 & 3.0 & 15.7 & 3.0\\\midrule
\multirow{2}{*}{$\varepsilon=2$} & \multicolumn{1}{c}{\scriptsize precision} & 22.3 & 11.9 & 15.5 & 5.8 & 12.4 & 3.0 & 11.3 & 2.2 & 10.0 & 1.5\\
& \multicolumn{1}{c}{\scriptsize recall} & 4.0 & 1.9 & 5.6 & 1.7 & 9.0 & 1.6 & 16.4 & 2.1 & 28.9 & 2.5\\\midrule
\multirow{2}{*}{$\varepsilon=3$} & \multicolumn{1}{c}{\scriptsize precision} & 27.5 & 7.7 & 25.3 & 4.9 & 24.6 & 5.4 & 22.6 & 3.2 & 20.3 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 5.0 & 1.1 & 9.2 & 1.3 & 17.8 & 2.7 & 32.9 & 2.6 & 59.2 & 3.7\\\midrule
\multirow{2}{*}{$\varepsilon=4$} & \multicolumn{1}{c}{\scriptsize precision} & 38.7 & 8.9 & 36.9 & 5.9 & 37.6 & 4.5 & 39.4 & 3.4 & 29.8 & 1.9\\
& \multicolumn{1}{c}{\scriptsize recall} & 7.0 & 1.3 & 13.5 & 1.8 & 27.4 & 1.8 & 57.4 & 1.3 & 86.9 & 2.2\\\midrule
\multirow{2}{*}{$\varepsilon=5$} & \multicolumn{1}{c}{\scriptsize precision} & 55.9 & 5.4 & 57.5 & 3.3 & 59.6 & 2.5 & 56.1 & 2.9 & 32.2 & 2.4\\
& \multicolumn{1}{c}{\scriptsize recall} & 10.2 & 0.7 & 21.0 & 0.7 & 43.6 & 1.7 & 81.9 & 2.9 & 93.8 & 1.2\\\midrule
\multirow{2}{*}{$\varepsilon=6$} & \multicolumn{1}{c}{\scriptsize precision} & 71.9 & 2.9 & 76.8 & 1.6 & 78.1 & 2.2 & 59.1 & 4.2 & 32.7 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 13.1 & 0.6 & 28.1 & 1.5 & 57.1 & 2.6 & 86.2 & 1.5 & 95.4 & 0.8\\\midrule
\multirow{2}{*}{$\varepsilon=7$} & \multicolumn{1}{c}{\scriptsize precision} & 88.1 & 2.1 & 88.7 & 1.5 & 86.0 & 2.1 & 61.9 & 3.7 & 33.5 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 16.1 & 0.8 & 32.5 & 1.8 & 63.0 & 3.2 & 90.3 & 1.2 & 97.6 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=8$} & \multicolumn{1}{c}{\scriptsize precision} & 94.0 & 0.8 & 93.5 & 0.5 & 88.4 & 1.7 & 63.4 & 3.5 & 33.8 & 2.2\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.2 & 1.2 & 34.3 & 2.3 & 64.7 & 3.4 & 92.6 & 1.7 & 98.5 & 0.6\\\midrule
\multirow{2}{*}{$\varepsilon=9$} & \multicolumn{1}{c}{\scriptsize precision} & 96.8 & 0.3 & 95.6 & 0.8 & 89.0 & 1.9 & 63.3 & 3.8 & 33.7 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.7 & 1.3 & 35.0 & 2.4 & 65.2 & 3.3 & 92.4 & 1.1 & 98.4 & 0.5\\\midrule
\multirow{2}{*}{$\varepsilon=10$} & \multicolumn{1}{c}{\scriptsize precision} & 97.5 & 0.4 & 96.3 & 0.3 & 89.4 & 1.7 & 62.8 & 4.2 & 33.5 & 2.3\\
& \multicolumn{1}{c}{\scriptsize recall} & 17.9 & 1.3 & 35.3 & 2.5 & 65.5 & 3.7 & 91.6 & 1.3 & 97.8 & 0.4\\
\bottomrule
    \end{tabular}%
}

\end{subtable}
\end{table}

}




==> tables/tab_attack_nonprivate_full.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[]
    \centering
    \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    \sisetup{detect-weight,mode=text,group-minimum-digits = 4}

    \caption{\small \textbf{Attack Performance} of \linkteller on different datasets, compared with two baseline methods LSA2-\{post, attr\}~\cite{he2020stealing}. Each table corresponds to a dataset. We sample nodes of low, unconstrained, and high degrees as our targets. Groups of rows represent different \textit{density belief} $\hat k$ of the attacker.
    % We examine three different sampling scenarios, constituting three column groups in the table. Each row corresponds to one belief on the \small ratio of edges. 
    % Results are reported over three runs.
    }
    % \vspace{-4mm}
    \label{tab:att-np}



\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{twitch-RU}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 33.0 & 2.8  & \bfseries 95.1 & 1.1  & \bfseries 26.0 & 1.0  & \bfseries 98.9 & 0.2  & \bfseries 18.1 & 1.3 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.2 & 0.3  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 1.3 & 0.5  & 0.4 & 0.1  & 2.5 & 1.3  & 0.4 & 0.2 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 61.3 & 5.1  & \bfseries 87.9 & 0.4  & \bfseries 48.1 & 2.3  & \bfseries 97.1 & 0.3  & \bfseries 35.6 & 2.6 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.2  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 1.7 & 0.2  & 0.9 & 0.1  & 2.5 & 0.5  & 0.9 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 78.7 & 1.9  & \bfseries 92.6 & 5.5  & \bfseries 71.8 & 2.2  & \bfseries 78.5 & 2.4  & \bfseries 89.7 & 1.7  & \bfseries 65.7 & 3.9 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.1  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 1.1 & 0.1  & 1.2 & 0.1  & 2.2 & 0.6  & 1.6 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 42.7 & 3.4  & \bfseries 100.0 & 0.0  & \bfseries 43.5 & 1.9  & \bfseries 95.0 & 0.5  & \bfseries 62.9 & 4.2  & \bfseries 91.8 & 1.3 \\
            & LSA2-post  & 0.7 & 0.9  & 1.8 & 2.5  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1 \\
            & LSA2-attr  & 1.3 & 0.9  & 3.2 & 2.3  & 0.8 & 0.1  & 1.8 & 0.3  & 2.0 & 0.3  & 2.8 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 21.3 & 1.7  & \bfseries 100.0 & 0.0  & \bfseries 22.5 & 1.1  & \bfseries 98.1 & 0.6  & \bfseries 33.6 & 2.5  & \bfseries 98.0 & 0.4 \\
            & LSA2-post  & 0.3 & 0.5  & 1.8 & 2.5  & 0.0 & 0.0  & 0.1 & 0.1  & 0.0 & 0.0  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.7 & 0.5  & 3.2 & 2.3  & 0.7 & 0.1  & 3.0 & 0.5  & 1.6 & 0.3  & 4.6 & 0.5 \\\bottomrule
\end{tabular}%
}
\end{subtable}


\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{twitch-DE}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 83.3 & 23.6  & \bfseries 26.2 & 7.0  & \bfseries 94.0 & 1.3  & \bfseries 22.5 & 1.3  & \bfseries 99.0 & 0.4  & \bfseries 25.2 & 1.2 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.2  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.4 & 0.5  & 0.1 & 0.1  & 2.6 & 1.1  & 0.7 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 91.7 & 11.8  & \bfseries 55.2 & 3.7  & \bfseries 92.4 & 4.1  & \bfseries 44.2 & 1.6  & \bfseries 96.9 & 0.3  & \bfseries 49.2 & 2.5 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.1  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.9 & 0.3  & 0.4 & 0.1  & 2.5 & 0.8  & 1.3 & 0.5 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 81.8 & 4.8  & \bfseries 92.5 & 5.9  & \bfseries 81.2 & 6.6  & \bfseries 77.2 & 3.4  & \bfseries 79.2 & 1.1  & \bfseries 80.4 & 3.1 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 1.2 & 0.3  & 1.2 & 0.4  & 1.8 & 0.4  & 1.8 & 0.5 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 44.7 & 3.4  & \bfseries 95.2 & 6.7  & \bfseries 49.0 & 4.7  & \bfseries 93.1 & 3.2  & \bfseries 46.9 & 2.0  & \bfseries 95.0 & 0.9 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1  & 0.1 & 0.1  & 0.0 & 0.0  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.8 & 0.1  & 1.6 & 0.2  & 1.4 & 0.3  & 2.8 & 0.8 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 23.8 & 0.3  & \bfseries 100.0 & 0.0  & \bfseries 25.8 & 1.9  & \bfseries 98.1 & 0.7  & \bfseries 24.3 & 1.1  & \bfseries 98.5 & 0.5 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1  & 0.2 & 0.2  & 0.0 & 0.0  & 0.0 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.7 & 0.1  & 2.7 & 0.4  & 1.1 & 0.2  & 4.4 & 0.9 \\\bottomrule
\end{tabular}%
}
\end{subtable}


\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{twitch-FR}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 28.3 & 2.4  & \bfseries 97.2 & 0.9  & \bfseries 22.7 & 0.6  & \bfseries 99.4 & 0.5  & \bfseries 24.1 & 2.1 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.2 & 0.2  & 0.0 & 0.1  & 0.5 & 0.2  & 0.1 & 0.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.6 & 0.4  & 0.1 & 0.1  & 1.9 & 0.7  & 0.5 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 50.0 & 0.0  & \bfseries 95.0 & 1.0  & \bfseries 44.3 & 1.3  & \bfseries 98.3 & 1.0  & \bfseries 47.7 & 4.5 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.1  & 0.0 & 0.1  & 0.3 & 0.1  & 0.1 & 0.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.6 & 0.2  & 0.3 & 0.1  & 1.4 & 0.2  & 0.7 & 0.0 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 92.5 & 5.4  & \bfseries 92.5 & 5.4  & \bfseries 84.1 & 3.7  & \bfseries 78.2 & 1.9  & \bfseries 83.2 & 1.4  & \bfseries 80.6 & 6.7 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1  & 0.0 & 0.1  & 0.1 & 0.0  & 0.1 & 0.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.8 & 0.2  & 0.7 & 0.2  & 1.4 & 0.2  & 1.3 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 51.1 & 1.6  & \bfseries 100.0 & 0.0  & \bfseries 51.3 & 2.1  & \bfseries 95.3 & 1.3  & \bfseries 49.1 & 2.7  & \bfseries 94.8 & 3.2 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1  & 0.1 & 0.0  & 0.1 & 0.0 \\
            & LSA2-attr  & 1.7 & 2.4  & 3.3 & 4.7  & 0.8 & 0.1  & 1.4 & 0.2  & 1.6 & 0.2  & 3.1 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 25.6 & 0.8  & \bfseries 100.0 & 0.0  & \bfseries 26.5 & 1.1  & \bfseries 98.3 & 1.0  & \bfseries 25.4 & 1.8  & \bfseries 97.6 & 1.6 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1  & 0.0 & 0.0  & 0.1 & 0.0 \\
            & LSA2-attr  & 0.8 & 1.2  & 3.3 & 4.7  & 1.0 & 0.2  & 3.7 & 0.8  & 1.5 & 0.1  & 5.7 & 0.1 \\\bottomrule
\end{tabular}%
}
\end{subtable}


\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{twitch-ENGB}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 30.3 & 4.1  & \bfseries 92.6 & 3.0  & \bfseries 25.5 & 4.9  & \bfseries 98.8 & 0.5  & \bfseries 25.2 & 0.2 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.2  & 0.0 & 0.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.5 & 0.4  & 0.4 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 54.2 & 8.7  & \bfseries 84.3 & 5.6  & \bfseries 45.6 & 7.6  & \bfseries 96.0 & 1.2  & \bfseries 48.9 & 0.6 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.1  & 0.0 & 0.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.4  & 0.2 & 0.2  & 1.8 & 0.3  & 0.9 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 83.1 & 6.6  & \bfseries 84.0 & 11.4  & \bfseries 67.9 & 6.3  & \bfseries 72.9 & 10.9  & \bfseries 81.6 & 2.7  & \bfseries 83.1 & 2.7 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.0  & 0.1 & 0.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.7 & 0.2  & 0.7 & 0.2  & 2.0 & 0.1  & 2.0 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 50.7 & 8.2  & \bfseries 97.9 & 2.9  & \bfseries 43.6 & 9.0  & \bfseries 91.2 & 4.9  & \bfseries 47.3 & 0.7  & \bfseries 96.3 & 1.3 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.4 & 0.5  & 0.8 & 1.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.5 & 0.2  & 1.2 & 0.6  & 1.7 & 0.2  & 3.4 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 26.0 & 4.9  & \bfseries 100.0 & 0.0  & \bfseries 23.5 & 5.9  & \bfseries 97.3 & 1.1  & \bfseries 24.2 & 0.2  & \bfseries 98.5 & 0.5 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.2 & 0.2  & 0.8 & 1.0 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.4 & 0.2  & 1.7 & 1.0  & 1.7 & 0.1  & 6.9 & 0.3 \\\bottomrule
\end{tabular}%
}
\end{subtable}


\end{table}

\begin{table}[]
%     \centering
%     \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
%     \sisetup{detect-weight,mode=text,group-minimum-digits = 4}
%     \caption{\small \textbf{Attack Performance} of \linkteller (cont'd).
%     }
%     % \vspace{-4mm}
%     \label{tab:att-np-2}
\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{twitch-PTBR}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 26.7 & 1.3  & \bfseries 95.6 & 1.6  & \bfseries 25.1 & 6.5  & \bfseries 98.4 & 1.3  & \bfseries 24.2 & 2.5 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.1  & 0.0 & 0.0 \\
            & LSA2-attr  & 4.6 & 3.3  & 1.2 & 0.9  & 4.7 & 0.9  & 1.2 & 0.4  & 6.9 & 0.7  & 1.7 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 99.0 & 1.5  & \bfseries 52.3 & 3.3  & \bfseries 93.6 & 1.4  & \bfseries 49.0 & 12.0  & \bfseries 97.3 & 1.6  & \bfseries 47.9 & 4.7 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0 \\
            & LSA2-attr  & 2.4 & 1.7  & 1.2 & 0.9  & 4.4 & 0.8  & 2.3 & 0.8  & 6.3 & 1.0  & 3.0 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 85.4 & 2.2  & \bfseries 89.2 & 4.2  & \bfseries 78.7 & 8.7  & \bfseries 80.3 & 13.1  & \bfseries 86.0 & 5.8  & \bfseries 84.2 & 4.0 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0 \\
            & LSA2-attr  & 1.2 & 0.9  & 1.2 & 0.9  & 4.3 & 0.9  & 4.7 & 1.7  & 6.0 & 0.8  & 5.9 & 0.5 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 48.3 & 2.7  & \bfseries 100.0 & 0.0  & \bfseries 48.7 & 12.2  & \bfseries 95.7 & 4.1  & \bfseries 50.2 & 5.4  & \bfseries 97.9 & 0.4 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 2.4 & 1.7  & 4.7 & 3.2 \\
            & LSA2-attr  & 0.6 & 0.4  & 1.2 & 0.9  & 3.8 & 0.3  & 8.0 & 2.4  & 5.0 & 0.7  & 9.8 & 0.6 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 24.1 & 1.4  & \bfseries 100.0 & 0.0  & \bfseries 25.5 & 7.5  & \bfseries 99.0 & 0.6  & \bfseries 25.5 & 2.8  & \bfseries 99.5 & 0.1 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 1.3 & 0.9  & 6.5 & 4.7  & 2.5 & 0.2  & 10.1 & 1.9 \\
            & LSA2-attr  & 0.6 & 0.2  & 2.4 & 0.7  & 3.1 & 0.2  & 13.2 & 3.6  & 4.1 & 0.4  & 15.8 & 0.5 \\\bottomrule
\end{tabular}%
}
\end{subtable}


\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{PPI}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 26.1 & 2.2  & \bfseries 99.5 & 0.7  & \bfseries 25.9 & 2.7  & \bfseries 99.7 & 0.3  & \bfseries 21.6 & 0.8 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.4 & 0.6  & 0.3 & 0.1 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.3 & 0.7  & 0.3 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 100.0 & 0.0  & \bfseries 47.6 & 4.7  & \bfseries 99.5 & 0.8  & \bfseries 51.5 & 5.4  & \bfseries 99.7 & 0.2  & \bfseries 43.3 & 1.6 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.4  & 0.1 & 0.2  & 1.6 & 0.5  & 0.7 & 0.2 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.6 & 0.3  & 0.3 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 98.7 & 1.9  & \bfseries 89.2 & 7.9  & \bfseries 89.5 & 6.5  & \bfseries 91.9 & 3.7  & \bfseries 98.0 & 0.3  & \bfseries 85.1 & 3.2 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.2  & 0.3 & 0.2  & 2.1 & 0.6  & 1.8 & 0.6 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.2  & 0.1 & 0.2  & 0.3 & 0.2  & 0.3 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 56.7 & 6.6  & \bfseries 100.0 & 0.0  & \bfseries 49.0 & 5.4  & \bfseries 100.0 & 0.0  & \bfseries 57.7 & 2.3  & \bfseries 100.0 & 0.0 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.2  & 0.5 & 0.4  & 2.1 & 0.1  & 3.6 & 0.3 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.1 & 0.1  & 0.1 & 0.2  & 0.2 & 0.1  & 0.3 & 0.1 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 28.3 & 3.3  & \bfseries 100.0 & 0.0  & \bfseries 24.5 & 2.7  & \bfseries 100.0 & 0.0  & \bfseries 28.8 & 1.2  & \bfseries 100.0 & 0.0 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.1  & 1.3 & 0.3  & 2.0 & 0.0  & 7.0 & 0.1 \\
            & LSA2-attr  & 0.3 & 0.5  & 1.1 & 1.6  & 0.0 & 0.0  & 0.1 & 0.2  & 0.1 & 0.0  & 0.3 & 0.1 \\\bottomrule
\end{tabular}%
}
\end{subtable}


\begin{subtable}[]{\columnwidth}
    \centering
    \vspace{0.5em}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{cc
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
  S[table-format=3.1]
  @{\tiny${}\pm{}$}
  >{\tiny}S[table-format=2.1]<{\endcollectcell}
}
    \toprule
    \multicolumn{2}{c}{\textbf{Flickr}} &  \multicolumn{4}{c}{\small low}  & \multicolumn{4}{c}{\small unconstrained} & \multicolumn{4}{c}{\small high}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \makecell{\small $\hat k$} & Method   & \multicolumn{2}{c}{\small precision}  & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} & \multicolumn{2}{c}{\small precision} & \multicolumn{2}{c}{\small recall} \\\midrule
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/4$}}
            & Ours  & \bfseries 83.3 & 23.6  & \bfseries 26.1 & 5.5  & \bfseries 63.9 & 30.7  & \bfseries 18.4 & 9.0  & \bfseries 14.9 & 3.8  & \bfseries 3.8 & 1.3 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.4 & 2.0  & 0.4 & 0.6 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.7 & 1.0  & 0.2 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k/2$}}
            & Ours  & \bfseries 63.9 & 10.4  & \bfseries 38.3 & 10.3  & \bfseries 60.0 & 22.5  & \bfseries 29.7 & 11.7  & \bfseries 19.6 & 2.8  & \bfseries 9.9 & 1.9 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.8 & 1.1  & 0.9 & 0.6 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.4 & 0.5  & 0.2 & 0.3 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$k$}}
            & Ours  & \bfseries 51.0 & 7.0  & \bfseries 53.3 & 4.7  & \bfseries 33.8 & 13.3  & \bfseries 32.1 & 13.3  & \bfseries 18.2 & 4.5  & \bfseries 18.5 & 6.1 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 2.3 & 0.7  & 2.3 & 0.9 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.4  & 0.3 & 0.4 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$2k$}}
            & Ours  & \bfseries 34.5 & 6.7  & \bfseries 71.1 & 15.0  & \bfseries 27.3 & 8.4  & \bfseries 50.3 & 16.8  & \bfseries 13.3 & 1.7  & \bfseries 26.8 & 5.6 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.6 & 0.6  & 3.2 & 1.3 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.4 & 0.4  & 0.8 & 0.9 \\[0.05em]\midrule[0.05em]
\rowcolor{tabgray}
\cellcolor{white}{\multirow{3}{*}{$4k$}}
            & Ours  & \bfseries 21.7 & 2.4  & \bfseries 86.1 & 10.4  & \bfseries 19.8 & 3.0  & \bfseries 71.9 & 10.6  & \bfseries 9.2 & 0.8  & \bfseries 37.3 & 7.1 \\
            & LSA2-post  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 1.3 & 0.3  & 5.3 & 1.2 \\
            & LSA2-attr  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.3 & 0.2  & 1.3 & 0.9 \\\bottomrule
\end{tabular}%
}
\end{subtable}

\end{table}
}
